Multi-Agent Reinforcement Learning with Multi-Step Generative Models

We consider model-based reinforcement learning (MBRL) in 2-agent, high-fidelity continuous control problems -- an important domain for robots interacting with other agents in the same workspace. For non-trivial dynamical systems, MBRL typically suffers from accumulating errors. Several recent studies have addressed this problem by learning latent variable models for trajectory segments and optimizing over behavior in the latent space. In this work, we investigate whether this approach can be extended to 2-agent competitive and cooperative settings. The fundamental challenge is how to learn models that capture interactions between agents, yet are disentangled to allow for optimization of each agent behavior separately. We propose such models based on a disentangled variational auto-encoder, and demonstrate our approach on a simulated 2-robot manipulation task, where one robot can either help or distract the other. We show that our approach has better sample efficiency than a strong model-free RL baseline, and can learn both cooperative and adversarial behavior from the same data.

==> formulation.tex <==
Let us first consider the single agent scenario.
Consider the following continuous control problem:
\begin{equation*}
    \begin{split}
        \max_{u_0,\dots,u_T} & \sum c(x_t,u_t) \\
        s.t. & \quad x_{t+1} = f(x_t, u_t)
    \end{split}
\end{equation*}
We denote $C(x_0,u_0,\dots,u_T) = \sum c(x_t,u_t)$.
Now, assume we have some model for the trajectory with a parameter $z$, that is, we can write
\begin{equation*}
    x_0,u_0,\dots,u_T = G(z),
\end{equation*}
for some $z$, for any $x_0,u_0,\dots,u_T$.
Then, an equivalent optimization problem is 
\begin{equation*}
    \max_z C(G(z)).
\end{equation*}
Note that there is no restriction on the model here, except that there is a one-to-one mapping between the trajectory and $z$. In particular, the single step model fits this derivation, where in that case $z$ would trivially correspond to the sequence of actions $u_0,\dots,u_T$. However, when we learn the model from data, it might be that we want different representations.

Now, let's consider the two-player game setting, where we are interested in a max-min game.
\begin{equation}\label{eq:prob_uw}
    \begin{split}
        \max_{u_0,\dots,u_T} \min_{w_0,\dots,w_T}& \sum c(x_t,y_t,u_t,w_t) \\
        s.t. & \quad x_{t+1}, y_{t+1} = f(x_t, y_t, u_t, w_t).
    \end{split}
\end{equation}
We denote $C(x_0,y_0,u_0,w_0,\dots,u_T,w_T) = \sum c(x_t,y_t,u_t,w_t)$. Again, assume we have some model for the trajectory with a parameters $z_x,z_y$, that is, we can write
\begin{equation*}
    x_0,y_0,u_0,w_0,\dots,u_T,w_T = G(z_x,z_y).
\end{equation*}
In addition, assume that $z_y$ is independent of $u_0,\dots,u_T$. That is, $\frac{\partial u_0,\dots,u_T}{\partial z_y} = 0$, and similarly $z_x$ is independent of $w_0,\dots,w_T$.
Then we can optimize
\begin{equation}\label{eq:prob_z}
    \max_{z_x} \min_{z_y} C(G(z_x, z_y)).
\end{equation}
This is justified as follows. A saddle point of \eqref{eq:prob_z} satisfies $\frac{\partial C}{\partial z_x} = 0$ and $\frac{\partial C}{\partial z_y} = 0$. We will show that it is also a saddle point of \eqref{eq:prob_uw}. We have that
\begin{equation*}
    \frac{\partial C}{\partial z_y} = \frac{\partial C}{\partial u_0,\dots,u_T} \frac{\partial u_0,\dots,u_T}{\partial z_y} + \frac{\partial C}{\partial w_0,\dots,w_T} \frac{\partial w_0,\dots,w_T}{\partial z_y},
\end{equation*}
and therefore 
\begin{equation*}
    \frac{\partial C}{\partial w_0,\dots,w_T} \frac{\partial w_0,\dots,w_T}{\partial z_y} = 0.
\end{equation*}
So long as $z_y$ is not redundant, i.e., $\frac{\partial w_0,\dots,w_T}{\partial z_y}\neq 0$, we have that $\frac{\partial C}{\partial w_0,\dots,w_T}=0$. Following the same derivation for $z_x$, we obtain a saddle point for \eqref{eq:prob_uw}.



==> main_icml.tex <==
% \documentclass{article}

% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{color}
\usepackage{subcaption}
\usepackage{booktabs} % for professional tables

% hyperref makes hyperlinks in the resulting PDF.
% If your build breaks (sometimes temporarily if a hyperlink spans a page)
% please comment out the following usepackage line and replace
% \usepackage{icml2019} with \usepackage[nohyperref]{icml2019} above.
\usepackage{hyperref}

% Attempt to make hyperref and algorithmic work together better:
\newcommand{\theHalgorithm}{\arabic{algorithm}}

% Use the following line for the initial blind version submitted for review:
% \usepackage{icml2019}

% If accepted, instead use the following line for the camera-ready submission:
\usepackage[accepted]{icml2019}

\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{tabularx}

%%% Comments
\newcommand{\mycomm}[3]{{\color{#2} \textbf{[#1: #3]}}} 
%define your comment NAME and COLOR here
\newcommand{\AT}[1]{\mycomm{AT}{magenta}{#1}}
\newcommand{\OK}[1]{\mycomm{OK}{cyan}{#1}}

% The \icmltitle you define below is probably too long as a header.
% Therefore, a short form for the running title is supplied here:
\icmltitlerunning{Multi Agent Reinforcement Learning with Multi-Step Generative Models}

\begin{document}

\twocolumn[
\icmltitle{Multi Agent Reinforcement Learning with Multi-Step Generative Models}

\icmlsetsymbol{equal}{*}

\begin{icmlauthorlist}
\icmlauthor{Orr Krupnik}{tec}
\icmlauthor{Igor Mordatch}{opi}
\icmlauthor{Aviv Tamar}{tec}
\end{icmlauthorlist}

\icmlaffiliation{tec}{Technion, Israel Institute of Technology, Haifa, Israel}
\icmlaffiliation{opi}{OpenAI}

\icmlcorrespondingauthor{Orr Krupnik}{ok1@campus.technion.ac.il}

\icmlkeywords{Machine Learning, ICML}

\vskip 0.3in
]

% this must go after the closing bracket ] following \twocolumn[ ...

% This command actually creates the footnote in the first column
% listing the affiliations and the copyright notice.
% The command takes one argument, which is text to display at the start of the footnote.
% The \icmlEqualContribution command is standard text for equal contribution.
% Remove it (just {}) if you do not need this facility.

\printAffiliationsAndNotice{}  % leave blank if no need to mention equal contribution
% \printAffiliationsAndNotice{\icmlEqualContribution} % otherwise use the standard text.

\begin{abstract}
The dynamics between agents and the environment are an important component of multi-agent Reinforcement Learning (RL), and learning them provides a basis for decision making. However, a major challenge in optimizing a learned dynamics model is the accumulation of error when predicting multiple steps into the future. 
Recent advances in variational inference provide model based solutions that predict complete trajectory segments, and optimize over a latent representation of trajectories. For single-agent scenarios, several recent studies have explored this idea, and showed its benefits over conventional methods. In this work, we extend this approach to the multi-agent case, and effectively optimize over a latent space that encodes \emph{multi-agent strategies}. We discuss the challenges in optimizing over a latent variable model for multiple agents, both in the optimization algorithm and in the model representation, and propose a method for both cooperative and competitive settings based on risk-sensitive optimization. We evaluate our method on tasks in the multi-agent particle environment and on a simulated RoboCup domain.
\end{abstract}

\section{Introduction}
Many real world problems where multiple agents operate in the same environment can be cast as multi-agent systems. Examples include autonomous vehicles \cite{lee2017desire,chen2017socially,schmerling2017multimodal}, navigation in environments with humans \cite{ivanovic2018generative}, learning communication between agents \cite{mordatch2017emergence}, and multiplayer games \cite{stone2000layered,silver2016mastering}. 

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.22\textwidth}
        \includegraphics[width=\textwidth]{strat12.png}
        \caption{Single player offense}
        \label{fig:strat_alone}
    \end{subfigure} \hspace{0.02\textwidth}
    \begin{subfigure}[b]{0.22\textwidth}
        \includegraphics[width=\textwidth]{strat15.png}
        \caption{Passing players}
        \label{fig:strat_pass}
    \end{subfigure}
    % \framebox[\columnwidth]{\rule{0pt}{160pt}}
    \caption{Learning trajectory representations at the strategy level. We plot the trajectories predicted for two random latent variable draws in the RoboCup domain. Blue and cyan lines denote the two offense players (controlled by the agent) and red lines denote the defense players. The purple line denotes the ball. Trajectories are divided into segments of 10 time steps, and circles indicate segment starting points. In~(a) the agent plans a strategy where the blue player advances alone and shoots the ball from the left. In~(b) the strategy is different, and incorporates blue catching the ball and passing it to cyan. }
    \label{fig:hfo_strategies}
\end{figure}

In recent years, following advances in deep learning and reinforcement learning (RL) in particular \cite{sutton1998reinforcement}, there have been many attempts to apply RL to multi-agent domains. 
Research in RL can be classified into two main approaches: model-free RL and model-based RL. In model-free RL, agents attempt to learn a policy -- a mapping directly from states to actions, tuned to solve a specific task \cite{sutton1998reinforcement}. In model-based RL, learning techniques are applied to model the dynamics governing the environment. The learned model is then used for planning, enabling control in tasks for which agents were not specifically trained. In addition, model-based approaches are generally more sample efficient, thus converging faster and saving time when training RL agents in complex environments \cite{deisenroth2011pilco,kurutach2018model}. Finally, model-based methods are interpretable -- it is relatively easy to roll out a trajectory using a learned model, and analyze the knowledge encoded in it. In light of these benefits, this work focuses on model-based RL.

The application of model-based RL to complex, multi-agent domains presents significant challenges. 
% A major one lies in the way the model is learned. 
The typical approach for model learning involves predicting a single next state conditioned on past states and actions \cite{abbeel2005learning}. This method has some significant drawbacks, such as tending to accumulate error when rolled out multiple time steps into the future. 
% This typically occurs from accumulation of small errors at each step, or divergence from the distribution of states and actions explored during training, for example, when a collision occurs in a robotic domain \cite{mishra2017prediction}. 
When the dynamics are stochastic or the observation is noisy, both in single agent and multi-agent environments, this problem amplifies.

While multi-agent RL is difficult, game theory provides many guaranteed ways to solve multi-agent problems~\cite{cesa2006prediction}, but has mostly been studied in a `strategy space' formulation, where single actions are played against other agents, e.g. in matrix games. The aim of our work is to combine such strategic decision making into high-fidelity problems that can be captured by RL formulations, such as continuous control domains.

%%AT: here we need a paragraph about trajectory prediction models. 
For single-agent model-based RL, several recent studies proposed to mitigate the error accumulation problem by learning deep generative models of multi-step trajectory segments~\cite{mishra2017prediction,ke2018modeling,hafner2018learning,rhinehart2018deep}. Here, we collectively refer to these methods as \emph{multi-step generative models}. The idea in these approaches is to learn a distribution of future trajectory segments in an unsupervised manner, using a deep generative model (e.g. a VAE, \citealt{kingma2013auto}), and perform planning by searching in the latent space of the model.
% use some form of variational inference \cite{kingma2013auto} to embed future segments of multiple time steps in a low-dimensional latent space. 
In essence, the latent space captures a compact `strategy space' of the agent, and it has been shown that optimization over this latent space is more effective than optimizing over single-step actions. 

% This potentially avoids the error accumulation of iteratively rolling out one-step predictions, and has been shown to be more effective than optimizing over single-step actions. 
% The latent space can capture a compact 'strategy space' of the agent, and it has been shown that optimization over this latent space is more effective than optimizing over single-step actions. 
% All the aforementioned works, however, address a relatively simple domain, with a single agent and very few environment elements. Therefore, they are not well suited to multi-agent scenarios. 

We propose to solve multi-agent problems more efficiently by extending multi-step generative models to domains with multiple agents. 
% cooperating or competing in various tasks. 
Our idea is that by training a generative model for predicting trajectories of several interacting agents, we can capture a lower dimensional, more generalized representation of the states and actions that are likely in the data, thus comprising a `strategy space' of agent interaction, which can then be optimized using game theoretic ideas. An illustrative example in the RoboCup domain~\cite{kitano1997robocup} is provided in Fig.~\ref{fig:hfo_strategies}: here, different values of the latent variables correspond to different offense strategies, and optimization can be performed in a high-level strategy space instead of using low-level actions. 

We present a practical algorithm for trajectory optimization of multiple agents based on risk-sensitive optimization, and discuss several approaches to modeling trajectories for multiple agents that comply with planning based on latent-space search. We show that our method can learn effective models for continuous multi-agent domains with complex dynamics, both in the multi-agent particle environment~\cite{lowe2017multi} and on a simulated RoboCup domain.

% We show that our method can learn effective models for continuous multi-agent domains with complex dynamics, both in the such as a simulated RoboCup domain.


% We present a practical algorithm for trajectory optimization of multiple agents based on risk-sensitive optimization, using multiple TSMs learned separately for different types of agents. We show that our method can learn effective models for continuous multi agent domains with complex dynamics, such as a simulated RoboCup domain.

% Additionally, while the models described above optimize over agent actions to select future segments, we propose to learn a model which ignores the actions and generates future segments of states directly from the latent space. This creates a more flexible and diverse world model, which in turn leads to a more diverse set of policies to optimize over, and finally better trajectories. 

% OK: The following two paragraphs are from the previous submission and probably don't fit in the new version 
% One approach which aims to tackle the problems with model-based RL described above is presented by \citet{mishra2017prediction}, where a Temporal Segment Model (TSM) was proposed. TSMs learn a model which embeds future segments of multiple states in a low-dimensional latent space using a conditional variational autoencoder \cite{kingma2013auto}. This potentially avoids the error accumulation of iteratively rolling out one-step prediction models. The latent space can capture a compact 'strategy space' of the agent, and it has been shown that optimization over this latent space is more effective than optimizing over single-step actions. \citet{mishra2017prediction} also proposed a deep generative model based on a WaveNet architecture \cite{van2016wavenet} designed for continuous control tasks. This approach has been shown to outperform the single-step baseline, as well as methods rolled out multiple timesteps into the future, and more sophisticated frameworks such as LSTMs. 


% The latent space provides us with a lower dimensional, more generalized representation of the states and actions that are likely in the data, thus comprising a 'strategy space' of the agents.

\section{Related Work}
Many approaches consider model-based RL in domains with complex, stochastic dynamics. Our work is inspired by the Temporal Segment Models (TSMs) developed by~\citet{mishra2017prediction} and more recent approaches~\cite{ke2018modeling,hafner2018learning} which use conditional variational autoencoder (CVAE) based dynamics models to predict multiple time steps into the future based on a previous segment of states and actions. The dynamics model is then used to optimize over agent trajectories for a specific task. A different approach is taken by  \citet{nagabandi2017neural}, who use neural network dynamics models, combined with Model Predictive Control (MPC) and model-free fine tuning to achieve effective control and stable gaits in the MuJoCo baseline environment. \citet{williams2017information} also use MPC to learn from a trained dynamics model, achieving high levels of performance on both simulated and actual hardware tasks. The models used, however, are single time-step, fully connected neural network models,
% \citet{deisenroth2011pilco} learn a Gaussian process dynamics model and exploit the learned uncertainty structure to mitigate the effect of error accumulation during planning. 
and all the approaches described above consider only a single agent. 

Recently, model based approaches have also been successfully used to \textit{predict} the behavior of multiple agents in both cooperative and competitive environments. Most of these owe their success to advances in deep variational inference \cite{kingma2013auto}. \citet{lee2017desire} predict vehicle trajectories in environments with multiple counterparts, such as other vehicles and pedestrians. \citet{ivanovic2018generative} and \citet{schmerling2017multimodal} use CVAEs to predict human behavior for human-robot interaction. \citet{zheng2016generating} use deep RNN models to recreate trajectories of a team of basketball players. They provide the interesting observation of interpreting a latent variable as a 'macro-goal', which controls the strategy of an agent for a given period of time. This is similar to our interpretation of the latent space as a 'strategy space' for the agent to optimize in. To the best of our knowledge, our attempt to use the deep generative model and the prediction of agent behavior to \emph{optimize} over trajectories for a given task in a multi-agent environment is, as of yet, a novel contribution. 

% Other methods for multi-agent RL follow a model-free approach. We include them here for completeness, however, we choose to focus on model-based methods in this work for their advantages described above.
% The 'Decentralized Actor, Centralized Critic' of \citet{lowe2017multi} has been highly successful in solving specific tasks in mixed cooperative and competitive environments, similar to the ones we examine in this work. \citet{yang2018mean} average over the effects surrounding entities have on the controlled agent in order to scale up Actor-Critic and Q-Learning algorithms to large numbers of agents. Recently, \citet{jaderberg2018human} trained multiple agents in a simulated Capture the Flag game, using population based learning.

\section{New Formulation}
\input{formulation.tex}

\section{Background}
Many dynamical systems can be described and analyzed as Markov Decision Processes (MDPs, \citealt{sutton1998reinforcement}). At each time step of an MDP, the system is in some state $x_t \in \mathcal{X}$ and agents can perform actions $u_t \in \mathcal{U}$, where $\mathcal{X}$ and $\mathcal{U}$ are the sets of all possible states and actions, respectively. The dynamics of the system are some function $f$ such that $x_{t+1} = f(x_t, u_t)$ (or some probability distribution $\mathcal{P}(x_{t+1} | x_t, u_t)$), governing the transitions from one state of the system to the next. Given a reward function $r(x)$, the typical goal is to maximize the expected sum of rewards $\mathbb{E}\left[\sum_{t=0}^T r(x_t)\right]$.\footnote{Other common criteria include discounted and episodic formulations~\cite{sutton1998reinforcement}. Our results can be easily extended to these cases.}

% In the RL setting, the dynamics are assumed to be unknown. Model-based RL approaches learn a model for the dynamics, and then solve for a policy which maximizes rewards. Since in an MDP each state is dependent only on the previous one, the traditional approach for modelling the dynamics of a system attempts to approximate the transition function $f$ (or probability $\mathcal{P}$) using some function approximator, such as a feed-forward neural network~\cite{hunt1992neural,depeweg2017learning}. 

\subsection{Multi-step Generative Models}
%TODO: Cite TSMs, PlaNet, R2P2 etc., explain the idea of predicting a segment instead of a single timestep to get more accurate trajectories. Discuss prediction using latent space, and maybe mention predicting states directly and not actions. 
% Also, make sure this isn't redundant of the realted work section. 
% Relevant pargraphs from the original "Temporal Segment Models" section copied below. 

The traditional approach for modelling dynamics attempts to approximate the transition function $f$~\cite{hunt1992neural,depeweg2017learning}. Multi-step generative models (such as \citealt{mishra2017prediction,rhinehart2018deep,ke2018modeling}) learn a more generalized form of the system dynamics. Consider segments (or "chunks") of $H$ past agent observations $X^-=\{x_{t-H+1},...,x_{t}\}$ and segments of future observations $X^+=\{x_{t+1},...,x_{t+H}\}$. Multi-step models learn a distribution $P(X^+|X^-)$ to predict the segment of future states based on past states, thus enabling consideration of delayed effects of previous actions and capturing longer temporal relations between states than a single-step model. 

In this work we focus on the Temporal Segment Models (TSMs) of \citet{mishra2017prediction}, but the ideas presented here can be generalized to other multi-step generative models. 
% Note that the original TSMs described by \citet{mishra2017prediction} condition the model on past and future actions, while \citet{ke2018modeling} and \citet{hafner2018learning} condition on segments of past actions. However, we choose to omit the actions here for simplicity and to match our modifications to the model, explained below. Although this approach poses a harder learning problem, compelling us to learn both the dynamics and the decision making processes of other agents, conditioning over states alone generalizes our model and renders it a simpler solution, relieving us of the need to provide precise actions for every agent in the system.
TSMs use a CVAE architecture~\cite{kingma2013auto}, where an encoder learns a distribution over a latent variable $Z$ conditioned on future observations: $\mathcal{Q}(Z|X^+)$, 
while a decoder reconstructs $X^+$: 
% conditioned on $X^-$ and a sample from the latent variable $Z$, 
$\hat X^+ = D(X^-,Z)$.
% , modelling the distribution $\mathcal{P}^{(x)}(X^+|X^-)$. 
The CVAE model encodes the input $X^+$ to obtain the parameters $\mu_Z, \sigma_Z$ of a Gaussian distribution for the latent variable. 
The optimization objective is then a variational lower bound of the data log likelihood~\cite{kingma2013auto}:
% , as described by eq.~\eqref{eq:elbo}:
\begin{equation}
    \begin{split}
    \mathcal{L} = \mathbb{E}_{Z\sim Q(Z|X^+)} &\left[\log P(X^+|X^-,Z)\right] - \\ &\mathcal{D}_{KL}\left[Q(Z|X^+)||P_{prior}(Z)\right],
    \end{split}
    \label{eq:elbo}
\end{equation}
where $P_{prior}(Z) = \mathcal{N}(0,I)$, and $P(X^+|X^-,Z) = \mathcal{N}(D(X^-,Z),I)$.
% where the prior is a normal distribution $P_{prior}(Z) = \mathcal{N}(0,I)$.
Each instance of the latent variable describes a segment of observations, and the decoder can be used as a generative stochastic dynamics model, to create future segments $\hat X^+$ using samples from the prior. 
% See figure~\ref{fig:arch_orig} for a general scheme of the model architecture.

% OK: The following is specific TSM, should probably move to our architecture section
% For the model to be able to capture temporal relations between observations, both encoder and decoder networks incorporate several layers of dilated causal convolutions, similar to the WaveNet architecture \cite{van2016wavenet} which has proven extremely successful in capturing temporal relations and generating future predictions of both audio and images. The dilation enables the network to capture a wider receptive field of observation history, using a relatively small number of layers. Being fully convolutional, the resulting CVAE is differentiable and can be trained with backpropagation, using the reparametrization trick described by \citet{kingma2013auto}. Networks based on dilated causal convolutions have recently been shown to train more efficiently than other sequential architectures, such as RNNs \cite{bai2018empirical}. 

One of the motivations for learning a dynamics model is to later use this model to solve the MDP problem. Assume that the total horizon of interest $T$ can be segmented to $k$ segments of length $H$. Then, the learned model for future segment distribution $\mathcal{P}^{(x)}(X^+|X^-,Z)$ can be rolled out $k$ times to produce a distribution for a $T$-length trajectory, which we denote as $\mathcal{P}^{(x)} (x_{t} \vert x_{0:t-1}, z^{(1:k)})$, where $z^{(1:k)}$ denotes $k$ samples of the latent variable $Z$.
\citet{mishra2017prediction} suggest the following trajectory optimization problem:\footnote{In the model of \citet{mishra2017prediction}, the latent space actually encoded an action distribution $\mathcal{P}^{(u)}(U^+|U^-,Z)$, and the optimization problem was of the form: 
$    \max_{z^{(1)},...,z^{(k)}} \mathbb{E} \left[ \sum_{t=1}^{T} r(x_{t},u_{t}) \right] \quad
    \textrm{s.t. } x_{t} \sim \mathcal{P}^{(x)} (x_{t} \vert x_{0:t-1}, u_t) ,
    u_{t} \sim \mathcal{P}^{(u)} (u_{t} \vert x_{0:t-1}, z^{(1:k)}).
$
Here, we present a similar optimization problem for a model that considers state trajectories without direct action encoding.
} 
\begin{equation}
    % \begin{split}
    \max_{z^{(1:k)}} \mathbb{E} \left[ \sum_{t=1}^{T} r(x_{t}) \right],\quad 
    \textrm{s.t. } x_{t} \sim \mathcal{P}^{(x)} (x_{t} \vert x_{0:t-1}, z^{(1:k)}).
    % \end{split}
    \label{eq:traj_opt_clean}
\end{equation}
Note that the optimization is over the latent space $Z$ -- the latent space of the agent trajectory. In this sense, we are optimizing over the possible strategies that the agent can perform, as displayed in the data used for training the model. Problem \eqref{eq:traj_opt_clean} can be solved using gradient descent.\footnote{The distribution $\mathcal{P}^{(x)}(X^+|X^-,Z)$ is typically represented as a neural network that encodes the mean of a Gaussian. Then, the expectation in \eqref{eq:traj_opt_clean} can be approximated with the deterministic prediction of the mean trajectory.}


\section{Multi-Agent Multi-Step Generative Models}
In this paper, we consider an extension to the MDP model for a multi-agent setting known as a Markov Game~\cite{littman2001value}. For simplicity, we present the case of two agents, but our results can easily be extended to more players (e.g. as described by \citealt{littman2001value}). 
Consider two agents $x$ and $y$ acting in a dynamic environment. At time-step $t$, the states of the agents are denoted by $x_t$ and $y_t$, respectively. The agents each select an action $a_t \in \mathcal{A}$ and $b_t \in \mathcal{B}$, out of their respective action sets. The dynamics of the environment are then governed by the distribution (or function) $\mathcal{P}(x_{t+1}, y_{t+1} \vert x_t, y_t, a_t, b_t)$, and the agents obtain rewards $r_x(x_t,y_t)$ and $r_y(x_t,y_t)$, respectively. This formulation can be used to define adversarial scenarios (e.g. by selecting zero sum rewards), cooperative scenarios (e.g. by selecting the same reward function for both agents), or various combinations thereof. To simplify our presentation, in this work we focus on the case of deterministic dynamics, given by $x_{t+1}, y_{t+1} = f(x_t, y_t, a_t, b_t)$.\footnote{An extension to stochastic dynamics can be done by adding another uncontrolled agent with action $c$ that represents noise, and writing the transition as $x_{t+1}, y_{t+1} = f(x_t, y_t, a_t, b_t, c_t)$. We leave a full investigation of stochastic dynamics to future work.}

In our setting, we consider a case where only agent $x$ is controlled, while the policy and reward driving agent $y$ are not known. In particular, we do not assume that $y$ has any fixed behavior. Our goal is to optimize the sum of rewards for agent $x$ in this case. In the remainder of this section, we first describe our optimization criterion, and later discuss how to learn suitable generative multi-step models in order to optimize it.

\subsection{Risk-Sensitive Optimization Formulation}\label{sec:risk}
To solve the multi-agent decision problem above, we propose to learn a probabilistic model for the \emph{possible} behaviors of $y$, 
% $\mathcal{P}(b|x,y)$, 
as seen in the data, and optimize a \emph{risk-sensitive} behavior policy for $x$, where the risk attitude would correspond to our belief about the nature of agent $y$'s policy. In particular, we consider the conditional value at risk measure (CVaR, a.k.a.~expected shortfall, \citealt{rockafellar2000optimization}). The CVaR at level $\alpha$\% of a random variable denotes the expectation of the variable on the worst (or best) $\alpha$\% of cases. Intuitively, as we optimize for the worst (best) cases, we take into consideration the adversarial (cooperative) nature of the other agents in the game. This statement has been made concrete by \citet{artzner1999coherent}. In this work, therefore, we opt to maximize the risk-averse CVaR of agent $x$'s sum of rewards:  $\mathbb{E}\left[\left.\sum_{t=0}^T r(x_t,y_t)\right|\sum_{t=0}^T r(x_t,y_t) \leq Q_\alpha\right]$, where $Q_\alpha$ denotes the $\alpha$-quantile of the sum of rewards, and the expectation is taken with respect to agent $y$'s behavior. 
% $\mathcal{P}(b|x,y)$. 
Note that when $\alpha=1$, we obtain the expected sum of rewards, while for $\alpha \to 0$ we optimize for the worst case. \footnote{To maximize a risk-seeking agent, we consider  $\mathbb{E}\left[\left.\sum_{t=0}^T r(x_t,y_t)\right|\sum_{t=0}^T r(x_t,y_t) \geq Q_\alpha\right]$. In this case, $\alpha=0$ corresponds to the expected sum of rewards, while for $\alpha \to 1$ we optimize for the best case.}

Solving the risk-averse optimization problem would correspond to planning for an adversarial $y$, while computing a risk-seeking behavior would correspond to the assumption that $y$ is cooperative. Solving for the expectation, in this case, would be a 'middle ground' between assuming that $y$ is adversarial or cooperative. We next discuss how to learn suitable models for the behavior of $y$.

\subsection{Multi-Agent Temporal Segment Models}\label{sec:matsm}
In the following, we extend the TSM (and general multi-step generative models) to the Markov game setting. 

As discussed above, for the risk-sensitive optimization criterion (and also for other traditional game theoretic formulations, \citealt{cesa2006prediction}) we require a model for the possible behaviors of $y$. For a single-step dynamics model, it is easy to learn the distribution of $y$'s actions from data. Recall, however, that the main motivation behind multi-step generative models is to eliminate the need to model the effect of single actions on the state, and instead model state trajectory segments for both agents.
% How then, could we learn a multi-step generative model that is compatible with the CVaR optimization criterion?

We begin with an important observation: in the standard TSM and MDP setting, we can interpret the latent variable $Z$ as a code for the sequence of actions in a segment $\{u_{t},...,u_{t+H-1}\}$. The reason is that any feasible trajectory $\{x_{t+1},...,x_{t+H}\}$ in the system can be realized by some sequence of actions, so a distribution on the trajectories can be represented by a distribution on the actions that induce them (as it is just a change of variables). 

To simplify notation, we restrict our presentation to optimizing a single segment. The extension to a full trajectory is done by rolling out several segments, as in Eq.~\ref{eq:traj_opt_clean}. Similarly to the definitions of $X^-$ and $X^+$, let $Y^-$ and $Y^+$ denote the segments of $H$ past and future observations for agent $y$. For a two player game, we would like to learn a generative model for the distribution $P(X^+,Y^+|X^-,Y^-)$ with two latent components, $Z$ and $W$, which correspond to the sequences of actions in a segment for agent $x$, $\{a_{t},...,a_{t+H-1}\}$, and agent $y$, $\{b_{t},...,b_{t+H-1}\}$, respectively. Such a representation would allow us to cast the trajectory optimization problem in a standard game theoretic formulation, where the spaces of $Z$ and $W$ denote the possible strategies for each agent. For the CVaR objective, we would have:
\begin{align}
    \begin{split}
    \max_{z} & \textrm{ CVaR} \left[ \sum_{t=1}^{H} r(x_{t},y_{t}) \right] \\
    \textrm{s.t. } &x_{t},y_{t} \sim P(X^+,Y^+|X^-,Y^-, z, w), \\
    & w \sim P_{prior}(W).
    \end{split}
    \label{eq:traj_opt_multi}
\end{align}
However, learning such a generative model is not trivial, since the contribution of each action sequence to agent trajectories in the segment depends also on the dynamical system $f$, which is not known in advance. In the rest of this section, we propose two approaches for overcoming this problem. The first is by learning disentangled latent representations, and the second is by learning conditional models, which we show are sufficient under certain assumptions.  

\subsubsection{Disentangled Multi-Step Generative Models} \label{sec:disentangled}
Latent spaces in multi-step generative models are generally unstructured \cite{mishra2017prediction,rhinehart2018deep}, and cannot be queried to control various aspects of the predicted segment. Here, we propose a representation where the elements of the latent space are \emph{disentangled} with respect to their effect on the two agents' strategies. That is, some elements in the latent space control the strategy of agent $x$, while other elements control the strategy of $y$.
% Such a "seperability" property would be extremely helpful when optimizing models for multiple agents, as each part of the latent space could be trained to control the future trajectories of different agents. 
% We borrow ideas from \citet{chen2016infogan} and \cite{klys2018learning}, where the latent spaces of generative models are partitioned to control various aspects of the generated output. 

To learn such a representation, we borrow ideas from \citet{chen2016infogan} and \citet{klys2018learning}, and propose to use the notion of mutual information to induce dependency between elements in the latent space and desired elements in the predicted trajectory. 

The mutual information between random variables $Q$ and $V$ is:
% \begin{equation*}
$
    I(Q;V) = H(Q) - H(Q|V) = H(V) - H(V|Q),
$
% \end{equation*}
where $H(Q)$ denotes the entropy of $Q$, and $H(Q|V)$ denotes the conditional entropy~\cite{cover2012elements}. Following the discussion above, to induce a disentangled latent representation for $X$ and $Y$ we would like to maximize the mutual information between $Z$ and $X$, and between $W$ and $Y$. We therefore propose the following loss function for training the generative model:
\begin{equation}\label{eq:loss_info}
    \min_\theta \mathcal{L} - \lambda_1 I(Z; X^+) - \lambda_2 I(W; Y^+)
\end{equation}
where $\mathcal{L} = \mathbb{E}_{Z,W\sim Q} \left[\log P(X^+,Y^+|X^-,Y^-,Z,W)\right] - \mathcal{D}_{KL}\left[Q(Z,W|X^+,Y^+)||P_{prior}(Z,W)\right]$ is the evidence lower bound~\cite{kingma2013auto}, and $\lambda_1>0$ and $\lambda_2>0$ are weights on the mutual information terms. To optimize \eqref{eq:loss_info} in practice, we use the lower bound proposed by \citet{chen2016infogan} We provide a full algorithm (Alg.~\ref{alg1}) in the supplementary material.
% and a part of the output future prediction, $X^+_1$ (completing the notation from the previous subsection). 
% Therefore, incorporating our variational lower bound from eq.~\eqref{eq:elbo}, the optimization objective of learning our model becomes: 
% \begin{align}
%     \min_\theta \mathcal{L} - \lambda I(Z_1, X^+_1) 
% \end{align}
% As noted by \citet{chen2016infogan}, in practice, maximizing the mutual information term directly is hard, since it requires access to the posterior $\mathcal{P}(Z|X^+)$. We can instead lower bound the information term using Variational Information Maximization \cite{agakov2004algorithm}. As shown by \citet{chen2016infogan}, the lower bound can be written as:
% \begin{align}
%     \begin{split}
%         L_I(f, Q) &= \mathbb{E}_{Z_1\sim P(Z_1),X^+_1\sim f(Z, X^-)}[\log Q(Z_1|X^+)] + H(Z_1) \leq \\ 
%         &\leq I(Z_1, f(Z, X^-)) = I(Z_1, X^+_1)  = H(z_1) - H(Z_1|f(Z, X^-))        
%     \end{split}
% \end{align}

\subsubsection{Conditional Multi-Step Generative Models} \label{sec:cond_msgm}
An alternative disentangled model representation can be obtained by conditioning. Since $P(X^+,Y^+|X^-,Y^-)=P(X^+|X^-,Y^-)P(Y^+|X^-,Y^-,X^+)$, we can learn two independent models: one for $P(X^+|X^-,Y^-)$ with a latent variable $Z$, and one for $P(Y^+|X^-,Y^-,X^+)$ with a latent variable $W$. Such will guarantee that the latent variables $Z$ and $W$ represent the strategies of $X$ and $Y$, respectively. However, such a formulation is not necessarily compatible with our CVaR optimization approach.

Since we are optimizing over $Z$, and $P(X^+|X^-,Y^-)$ does not depend on the value of $W$, we are effectively letting agent $x$ `play first', and choose its trajectory, while agent $y$ can only react to the trajectory of $x$ that has already been chosen.\footnote{Conversely, if we model the distribution as $P(Y^+|X^-,Y^-)P(X^+|X^-,Y^-,Y^+)$, we are giving an advantage to player $y$.} This gives a clear advantage to player $x$, which we demonstrate in our experiments in a scenario where players can block each other (see fig.~\ref{fig:bumpers}). 

However, the conditional representation is still appropriate under some conditions. Consider a system where the dynamics of the agents are independent, i.e., can be written as $x_{t+1} = f_x(x_t, a_t)$ and $y_{t+1} = f_y(y_t, b_t)$, while the coupling between the agents is realized only through the reward function $r(x,y)$. In such cases, learning two independent models for the agents is compatible with the CVaR optimization. While this representation is limited in its applicability, its simplicity is an advantage in practice and, as we show in our experiments, it is suitable for several interesting domains such as the RoboCup simulation.

% The below is math we wrote a few months ago, which may describe the model a little better than the paragraph below it (of course we'll still need the CVaR parts)
% Is the conditional model always enough? Can we think of a scenario where we need a shared model for different agents? \\
% $P(x,y) = P(x|y)P(y)$ \\

% \subsection{Information Theoretic Generative Models}
% Latent spaces in multi-step generative models are generally unstructured \cite{mishra2017prediction,rhinehart2018deep}, and cannot be queried to control various aspects of the predicted segment. Such a "seperability" property would be extremely helpful when optimizing models for multiple agents, as each part of the latent space could be trained to control the future trajectories of different agents. We borrow ideas from \citet{chen2016infogan} and \cite{klys2018learning}, where the latent spaces of generative models are partitioned to control various aspects of the generated output. 

% We propose to use the notion of mutual information \eqref{eq:mut_inf} to enforce a relation between parts of the latent space and parts of the output variable. A general definition of mutual information is given by: 
% \begin{align}
%     I(X;Y) = H(x) - H(X|Y) = H(Y) - H(Y|X)
% \end{align}
% Where $H(X)$ denotes the entropy of a random variable $X$, and $H(X|Y)$ denotes the conditional information. In our case, we'd like to maximize mutual information between a part of the latent space, denoted by $Z_1$, and a part of the output future prediction, $X^+_1$ (completing the notation from the previous subsection). Therefore, incorporating our variational lower bound from eq.~\eqref{eq:elbo}, the optimization objective of learning our model becomes: 
% \begin{align}
%     \min_\theta \mathcal{L} - \lambda I(Z_1, X^+_1) 
% \end{align}
% As noted by \citet{chen2016infogan}, in practice, maximizing the mutual information term directly is hard, since it requires access to the posterior $\mathcal{P}(Z|X^+)$. We can instead lower bound the information term using Variational Information Maximization \cite{agakov2004algorithm}. As shown by \citet{chen2016infogan}, the lower bound can be written as:
% \begin{align}
%     \begin{split}
%         L_I(f, Q) &= \mathbb{E}_{Z_1\sim P(Z_1),X^+_1\sim f(Z, X^-)}[\log Q(Z_1|X^+)] + H(Z_1) \leq \\ 
%         &\leq I(Z_1, f(Z, X^-)) = I(Z_1, X^+_1)  = H(z_1) - H(Z_1|f(Z, X^-))        
%     \end{split}
% \end{align}


% Currently, our agent predicts $X^+ \sim P(X^+|X^-, Y^-; Z)$ and the opponent predicts $Y^+ \sim P(Y^+|X^-, Y^-, X^+; W) = \frac{P(Y^+, X^+|X^-, Y^-; W)}{P(X^+|X^-, Y^-)} $


% Multi agent dynamics:
% $x_{t+1},y_{t+1} = f(x_t, y_t, u_t, v_t, w_t)$, where $w_t$ is noise. 
% This is equivalent to writing $P(x_{t+1},y_{t+1}|x_t, y_t, u_t, v_t)$. If $v_t \sim \pi_y$, then
% $P(x_{t+1},y_{t+1}|x_t, y_t, u_t) = \sum_{v_t}P(x_{t+1},y_{t+1}|x_t, y_t, u_t, v_t)\pi_y(v_t)$. 

% And $P(x_{t+1},y_{t+1}|x_t, y_t, u_t) = P(y_{t+1}|x_{t+1},x_t, y_t, u_t)P(x_{t+1}|x_t, y_t, u_t)$.

% Assuming that actions only control single agents, $P(y_{t+1}|x_{t+1},x_t, y_t, u_t) = P(y_{t+1}|x_{t+1},x_t, y_t)$, so 

% $$P(x_{t+1},y_{t+1}|x_t, y_t, u_t) = P(y_{t+1}|x_{t+1},x_t, y_t)P(x_{t+1}|x_t, y_t, u_t)$$
%%%%%%%%%%%%%%%%%

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.235\textwidth}
        \includegraphics[width=\textwidth]{cond_bumper.png}
        \caption{Conditional model}
        \label{fig:conditional}
    \end{subfigure} %\hspace{0.05\textwidth}
    \begin{subfigure}[b]{0.235\textwidth}
        \includegraphics[width=\textwidth]{dis_bumper.png}
        \caption{Disentangled model}
        \label{fig:disentangled}
    \end{subfigure}
    \caption{Comparison between disentangled and conditional models on box bumper domain. Blue agent ($x$) attempts to reach the target location below the horizontal obstacle (green circle), 
    % while receiving negative reward for leaving the play area, and 
    possibly being blocked by the red agent ($y$) in the narrow passage. Numbers indicate the segment order in time. Fig.~\ref{fig:conditional} shows a trajectory predicted by the conditional model. Since $x$ is independent of $y$, which only `responds' to its actions, the optimization cannot imagine a trajectory for which $x$ is blocked by $y$ en route to the goal, even in the worst case (risk-averse optimization). In fig.~\ref{fig:disentangled}, a sample is shown from the predictions of the disentangled model, where $x$ chooses to go left, since it assumes $y$ will block it in the right passage.}
    % $x$'s path and prevent it from receiving its reward.  } 
    \label{fig:bumpers}
    \vspace{-1em}
\end{figure}

\section{Model Architecture}

We now discuss the implementation details of our approach for solving the multi-agent problem defined above. In this section, we describe the data collection process, model architecture and training, and how we use the learned models for optimization in the latent space.

\subsection{Data Collection}
In this work, we follow the approach of \citet{mishra2017prediction}, and assume that data for training the dynamics model is generated from a predefined exploration policy. This policy should be diverse enough to `cover' the interesting strategies that the model can learn. For the multi-agent case, we assume that we have an exploration policy both for the agent $x$ and for the adversary $y$. 
% In many model-based RL studies, the policy that was learned by the model was used to generate additional data in an iterative optimization formulation~\cite{kurutach2018model}. We leave this study to future work, and 
We note that in our experiments, designing a suitable exploration policy was relatively straightforward, by stochastic action selection with some heuristic direction.

\subsection{Models and Training}
Following the two approaches described in Sec.~\ref{sec:matsm}, we train a separate TSM for each agent in the conditional model, and a shared TSM with a disentangled latent space for the disentangled model. All models are based on the architecture described by \citet{mishra2017prediction}, using CVAEs with dilated causal convolutions in both encoder and decoder. Full implementation details are in the supplementary material. 

% Recall that in our setting we have a controlled agent $x$ and a non-controlled agent $y$, which can act as an adversary to $x$. To capture this relationship between the agents, we allow the model for $y$ to observe the actions of the controlled agent $x$ in a non-causal manner (i.e. they 'respond' to the actions of other agents). This allows us to predict the possible reaction of $y$ to the strategy of $x$. Concretely, assume the segments of observations for the controllable agent are given by $X^-, X^+$ for past and future observations respectively, and the segments for the other agent are given by $Y^-, Y^+$. The decoder of the controllable agent predicts $\hat X^+ \sim \mathcal{P}(X^+|X^-, Y^-; Z)$ while the responsive model for the second agent predicts $\hat Y^+ \sim \mathcal{P}(Y^+|Y^-, X^-, X^+; W)$, where $Z$ and $W$ are the latent variables controlling both models, respectively. A more detailed comparison of the architectures can be found in the supplementary material. 
% To train our TSMs, we organize our data into consecutive past and future segments of both agents $(X^-, Y^-), (X^+, Y^+)$, and optimize the variational lower bound \eqref{eq:elbo} using the Adam optimizer. Full implementation details can be found in the supplementary material.  

\subsection{Multi-Agent Trajectory Optimization}

% As noted above, the motivation for learning a dynamics model is to later use this model to find an optimal solution for a task in the environment. 
% In addition, trajectory optimization is a useful tool for measuring the performance of our model. Poorly trained or insufficient models tend to produce predictions which are unrealistic in the real environment -- which leads to sub-optimal solutions of the optimization problem.

% Assume that the total horizon of interest $T$ can be segmented into $k$ segments of length $H$. Then, the learned models for future segment distributions $\mathcal{P}(X^+|X^-, Y^-; Z)$ and $\mathcal{P}(Y^+|Y^-, X^-, X^+; W)$ can be rolled-out $k$ times to produce a distribution for a $T$-length trajectory for both agents $x_0,y_0,\dots,x_{T},y_{T}$.
% For each $i \in 1,\dots, k$, we denote by $x^{+,i} = x_{i H : (i + 1) H - 1}$ and $x^{-,i} = x_{(i - 1)H:iH - 1}$ the $i^{\text{th}}$ future and past segments for agent $X$ in this rolled-out trajectory. Similarly, for the non-controlled agent $y$, we denote $y^{+,i} = y_{i H : (i + 1) H - 1}$ and $y^{-,i} = y_{(i - 1)H:iH - 1}$. We also denote by $z^{i}$ and $w^{i}$ the $i^{\text{th}}$ samples of the latent variables $Z$ and $W$ used to roll out each segment in the trajectory.

Recall that in our problem formulation, we seek to find a risk-sensitive policy against the probabilistic behavior of the opponent $y$ (see Sec.~\ref{sec:risk}). 
% Our idea is that the learned model for the non-controlled agent $\mathcal{P}(Y^+|Y^-, X^-, X^+)$ can be used to model the possible behaviors of $y$. 
Therefore, we propose the following trajectory optimization problem:
\begin{align} 
    \begin{split}
    \min_{z^{1},...,z^{k}} &\mathbb{E} \left[\left. \sum_{t=0}^{T} r_x(x_{t}, y_t) \right| \sum_{t=0}^{T} r_x(x_{t}, y_t) \leq Q_\alpha \right] \\
    \textrm{s.t. } &x^{+,i},y^{+,i} = f^{(x,y)}(x^{-,i}, y^{-,i}, z^{i}, w^{i}), \forall i\in 1,\dots,k\\
    % &y^{+,i} = f^{(y)} (y^{-,i}, x^{-,i}, x^{+,i}, w^{i}),\quad \forall i\in 1,\dots,k\\
    & w^{i} \sim \mathcal{P}_{prior}(W),\quad \forall i\in 1,\dots,k ,
    \end{split}
    \label{eq:opt_expected_adv}
    \raisetag{50pt}
\end{align}
The function $f^{(x,y)}$ denotes the CVAE decoder, and depends on the type of model used. 
For the disentangled model, it is the decoder for both $x$ and $y$, while for the conditional model, each agent has its own decoder (cf. Section \ref{sec:cond_msgm}).
Note that this is a formulation of problem~\eqref{eq:traj_opt_multi} for our case, with notation following the setting described in Sec.~\ref{sec:risk}. 
% This formulation works for both settings proposed in Sec.~\ref{sec:matsm}: when using conditional multi-step generative models, $f^{(x)}$ and $f^{(y)}$ are the decoders of two separate models, where the model for $y$ depends on future observations of $x$; while in the disentangled setting, $f^{(x)}$ and $f^{(y)}$ are both implemented by the same model, with $z$ and $w$ the disentangled parts of the same latent space.
% where $Q_\alpha$ denotes the $\alpha$-quantile of $\sum_{t=0}^{T} r_x(x_{t}, y_t)$.
% Note that here, compared to the original TSMs, we are optimizing over the the latent space of the controlled agent $x$, but \emph{marginalizing} over the latent space of the non-controlled agent $y$. By controlling the risk sensitivity, we can tune our belief towards $y$ -- a risk-averse attitude (i.e., a small $\alpha$) will assume that $y$ will act against us, while a risk seeking behaviour (which can be achieved by replacing $\leq$ with $\geq$ in the objective) assumes that $y$ will act in our favor. Setting $\alpha=1$ will result in an agent that optimizes against the expected behavior of $y$, as displayed in the collected data.

% Note also that this setup can be extended to any number of agents, with one agent responding with its 'best option' for the average trajectories of other agents. See the next section for examples of optimization using this paradigm. 

To practically solve problem \eqref{eq:opt_expected_adv}, we use a combination of sampling and gradient descent. It is well known that the CVaR (or the CVaR gradient) at level $\alpha$\% of a random variable $\Xi$ can be estimated by taking $m$ samples of $\Xi$, and averaging the smallest $\alpha$\% of the samples (or their gradient)~\cite{hong2009simulating}. Thus, we can replace the expectation in \eqref{eq:traj_opt_clean} with an average of the $\alpha$\% smallest values of $\sum_{t=0}^{T} r_x(x_{t}, y_t)$, where the sample comes from sampling the $w^{i}$ values from $\mathcal{P}_{prior}(W)$. This results in a deterministic optimization problem, which we can solve using gradient descent. In our implementation, we used Adam~\cite{kingma2014adam}, with multiple restarts from random initial values of $z^{1},...,z^{k}$, sampled from $\mathcal{P}_{prior}(Z)$. Detailed pseudocode is given in the supplementary material (see Alg.~\ref{alg2}).

\subsection{Trajectory Execution}\label{sec:traj_execution}

The trajectory optimization described above can only solve for a \emph{desired} trajectory in state space for our agent $x$. However, to execute the trajectory in the system, we need to select actions that `carry out' the imagined future steps. Here, we exploit the fact that in many systems, designing a tracking controller can be much simpler than designing a full policy~\cite{schaal2006dynamic}.

We propose to use the training data to also learn, in addition to the TSM models, an inverse dynamics model $P(u_t|x_t,x_{t+1})$. Using such a model, and the predicted state sequence for the agent $x_0,\dots,x_T$ (the result of trajectory optimization), we can compute actions that execute the desired trajectory.
Training an inverse dynamics model is a standard supervised learning problem, and in our experiments we found that standard multi-layered perceptrons (MLPs) work well.
To execute a full trajectory in the system, we adopt a model predictive control approach (MPC,~\citealt{nagabandi2017neural}): at the beginning of each segment $i$, we solve the trajectory optimization problem for the remaining segments $i,i+1,\dots,k$, starting from the current state of the agents, to obtain the desired trajectory for the agent at the current segment $x^{+,i}$. We then use the inverse model to track this trajectory segment. Then, at segment $i+1$, we observe the current position of the agents, solve the trajectory optimization again for the remaining $i+1,\dots,k$ segments, and repeat. This approach reduces the effect of drift from the imperfect inverse model, and also updates the controllable agent $x$'s policy against the real observations of the non-controlled agent $y$.

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.235\textwidth}
        \includegraphics[width=\textwidth]{temp_seg_7771.png}
        \caption{TSM trajectory (risk neutral)}
        \label{fig:tsm_traj}
    \end{subfigure} %\hspace{0.05\textwidth}
    \begin{subfigure}[b]{0.235\textwidth}
        \includegraphics[width=0.975\textwidth]{single_step_7771.png}
        \caption{Single step baseline}
        \label{fig:ssb_traj}
    \end{subfigure}
    \caption{Predator-Prey domain. The predator (blue) attempts to reach the escaping target (red) around the obstacle in the middle of the field.
    (a) Trajectory optimization for TSM using the risk-neutral setting ($\alpha=1$). (b) Trajectory optimization for the single step baseline. In both cases, the chasing agent (blue) starts to the left of the wall, while the target (red) starts to the right across from it. The trajectories are marked at every tenth step to enable temporal comparison, which coincides with the segment lengths for the TSM case. Both models imagine a successful chase of the prey. However, the TSM trajectory successfully circumvents the obstacle to reach the expected average location of the prey, while the baseline exploits an error in the the single step model and completely ignores the wall, which would fail at execution.} \label{fig:fc_traj_opt}
    \vspace{-1em}
\end{figure}

\section{Experiments}
To test our models, we use simulators and data collected from two domains:
% four multi-agent games. The first is a box environment, with one agent attempting to reach a goal location, while the other tries to block its path. The second and third tasks are set in a simple predator-prey scenario designed using
Multi-Agent Particle Environments -- a standard benchmark for multi-agent RL~\cite{lowe2017multi}, 
% A single agent tries to reach a target around an obstacle, while the target escapes in an adversarial manner. The fourth, more complex domain is
and 2D RoboCup Soccer Simulation \cite{kitano1997robocup,kalyanakrishnan2006half}.
% with two offensive players attempting to score against a defender and a goalkeeper.
% details for both of which are described below.

\subsection{Multi-Agent Particle Environments}\label{sec:particle}
Multi-Agent Particle Environments are a highly versatile RL playground, proposed by \citet{mordatch2017emergence} and used extensively in other work (e.g., \citealt{lowe2017multi}). The Particle Environment world allows for an arbitrary number of interacting agents, with user defined state and action spaces, and a highly configurable set of landmarks. For our experiments, we designed three simple environments: 

\textbf{(1)~Box-bumper:} a small, closed world where one agent attempts to reach a specified location behind an obstacle, while the other agent attempts to block it (see fig.~\ref{fig:bumpers}). 
\textbf{(2)~Predator-prey:} similarly to the scenario created by \citet{lowe2017multi}, a single agent chases an escaping target around an obstacle (see fig.~\ref{fig:fc_traj_opt}). Predator reward is negative distance to the prey.
% , while the prey attempts to maximize the same distance.
\textbf{(3)~Safe zone predator-prey:} modification of the previous environment, where prey has a `safe zone' at the bottom right corner of the game (see fig.~\ref{fig:fc_cvar})

The data we collected to train the world model for all multi-agent particle environment domains consists of 30k trajectories of 50 steps each, where the agent applies 5 steps in a random direction, then continues to move with inertia, selects a new direction and repeats. This type of exploration provides trajectories which are relatively evenly distributed around the playing field, along with a sizable percentage of collisions with the obstacles, which are important for learning an accurate world model.

\begin{table}
    \caption{Results (average distance to prey, lower is better) for predator-prey domain using a trajectory optimization policy. Each row represents a different initial setup of predator and prey relative to the wall obstacle. The results were obtained by averaging over 20 trajectories starting on the same side, and 60 from different locations on different sides. Our model outperforms the single-step baseline and the original exploration policy from both locations, with a larger advantage when the agents start on different sides of the wall (harder scenario). \\ }
    % \begin{tabular}{c|c||c|c|c}
    %  \textbf{Agent} & \textbf{Target} & \textbf{TSM} & \textbf{Single} & \textbf{Random} \\
    %  \textbf{Location} & \textbf{Location} &  & \textbf{Step} & \\
    %  \hline
    %  $[0.4, 0.3]$ & $[0.4, -0.3]$ & \textbf{0.7204} & 0.9223 & 1.5512 \\
    %  \hline
    %  $[-0.4, 0.0]$ & $[0.3, -0.1]$ & \textbf{0.8647} & 1.3451 & 1.8296 \\
    %  \hline
    %  $[0.2, 0.0]$ & $[-0.3, 0.3]$ & \textbf{0.9294} & 1.1825 & 1.6525 \\
    %  \hline
    %  $[0.2, 0.0]$ & $[-0.2, 0.0]$ & \textbf{1.0173} & 1.1551 & 1.6395 \\
    %  \hline
    %  $[0.4, 0.3]$ & $[-0.3, 0.2]$ & \textbf{0.9832} & 1.3319 & 1.7636
    %  \end{tabular}
    %  \label{tab:fc_opt_res}
    \begin{tabular}{c||c|c|c}
     \textbf{Locations} & \textbf{TSM (Ours,} & \textbf{Single} & \textbf{Random} \\
     \textbf{(Relative to wall)} & \textbf{risk neutral)} & \textbf{Step} & \\
     \hline
     Same side & \textbf{0.7204} & 0.9223 & 1.5512 \\
     \hline
     Different sides & \textbf{0.9486} & 1.2537 & 1.7213
     \end{tabular}
     \label{tab:fc_opt_res}
     \vspace{-2em}
\end{table}

\subsubsection{Box Bumper Domain}
The box bumper domain consists of a square playing area, with a horizontal wall set in the bottom half of the field. Two agents, which are relatively large compared to the area of interest, move around the field by applying forces in one of the four cardinal directions. Due to the limited size of this domain, the agents tend to collide often and block each other's way. 
%% OK: we can move this to the supplementary
% In this domain, we used the data collection policy described above, modified such that the random direction selection is weighted towards the location of the other agent to promote collisions between the agents, which are an area of interest in the state space.
The task of one agent in this environment is to reach the goal location, which is located below the middle of the wall. The other agent may attempt to block its path. 

The experiments in this domain are qualitative in nature, and serve as an example to the case where the conditional multi-step generative model (see Sec.~\ref{sec:cond_msgm}) may not be suitable, and the disentangled models (see Sec.~\ref{sec:disentangled}) may be necessary for a correct solution. We trained two multi-agent TSMs on this domain: the first was trained in the conditional form, where one controlled agent attempts to reach the goal, and the second agent plans trajectories conditioned on the path of the first; a second, disentangled model was trained using the mutual information maximization technique. 
%% OK: supplementary
% The observation space included the locations and velocities of both agents.
Fig.~\ref{fig:bumpers} presents the results of trajectory prediction using both models.

\begin{figure}
    \centering
    % \begin{subfigure}[b]{0.23\textwidth}
    %     \includegraphics[width=\textwidth]{pess773p.png}
    %     \caption{TSM trajectory (risk averse)}
    %     \label{fig:pessTSM}
    % \end{subfigure}
    % \begin{subfigure}[b]{0.23\textwidth}
    %     \includegraphics[width=\textwidth]{opt776p.png}
    %     \caption{TSM trajectory (risk seeking}
    %     \label{fig:optTSM}
    % \end{subfigure}
    \includegraphics[width=0.48\textwidth]{opt-pess_same_scale.png}
    \caption{Predator-Prey domain, with a safe zone for prey. The predator agent (blue, starts to the left of the obstacle) attempts to reach the prey (red, starts to the right), while the prey has a `safe zone' (marked by the green box) where the predator gets no reward for capturing it (and consequentially, the prey's reward grows). 
    Left: A risk-averse optimization, selecting the worst-case target trajectories and therefore anticipating that the prey goes towards the safe zone. Right: An optimistic optimization, where the best case prey trajectory moves away from the safe zone. } \label{fig:fc_cvar}
    % \vspace{-3em}
\end{figure}

\subsubsection{Predator-Prey}\label{sec:pred_prey}
The predator-prey domain simulates a chase scenario, with one agent chasing the other around a vertical wall obstacle. The cost incurred by the agent is the sum of distances between the agent and target along a complete trajectory.
%% OK: supplementary
% The observation space for each agent consists of the agent location, its velocity and the vector from the agent to the center of the wall. 
% We used the same learned model for both agents $x$ and $y$ when conducting trajectory optimization.

Data was collected with the exploration policy described above. Using the collected data, we trained two world models: a TSM and a single-step MLP dynamics model to serve as a baseline for comparison. We used both learned models to optimize over trajectories as described above (see Alg.~\ref{alg2} in the supplementary material). Despite exploring multiple network architectures and conducting a hyper-parameter search, none of the single step baselines we trained were able to correctly predict collisions with the wall. This enabled the baseline agent to exploit the failures of the model when optimizing for the best trajectories, as can be seen in fig.~\ref{fig:fc_traj_opt}. The same figure shows the success of our model in the same case. We compared the models quantitatively by executing their optimized trajectories in the simulator using MPC, playing against a target which used the aforementioned exploration policy. A comparison of the performance of the different models can be seen in Table~\ref{tab:fc_opt_res}.

\begin{table}
    \centering
    \caption{Results (average distance considering safe zone, lower is better) for the safe-zone predator-prey domain. The comparison was made by playing 100 scenarios starting from random starting locations, and averaged over 3 random seeds. \\}
    \begin{tabular}{c||c}
     \textbf{Optimization Method} & \textbf{Cost} \\
     \hline
     Risk averse (Worst case) & \textbf{0.9647} \\ %0.9682, 0.9358, 0.9894 
     \hline
     Risk neutral (average) & 1.0574 % 1.0508, 1.0689, 1.0452
     \end{tabular}
     \label{tab:fc_cvar}
\end{table}
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.22\textwidth}
        \includegraphics[width=0.85\textwidth]{real3.png}
        \caption{Baseline: captured ball}
        \label{fig:real3}
    \end{subfigure} %\hspace{0.05\textwidth}
    \begin{subfigure}[b]{0.22\textwidth}
        \includegraphics[width=0.85\textwidth]{imagined3.png}
        \caption{Predicted: goal}
        \label{fig:im3}
    \end{subfigure}
    \begin{subfigure}[b]{0.22\textwidth}
        \includegraphics[width=0.85\textwidth]{real15.png}
        \caption{Baseline: out of time}
        \label{fig:real15}
    \end{subfigure} %\hspace{0.05\textwidth}
    \begin{subfigure}[b]{0.22\textwidth}
        \includegraphics[width=0.85\textwidth]{imagined15.png}
        \caption{Predicted: goal}
        \label{fig:im15}
    \end{subfigure}
    \caption{Trajectory optimization in the HFO domain. Trajectories (a) and (c) are real trajectories of the hand coded Agent2D, while (b) and (d) are the respective optimized trajectories predicted by our model. Blue and Cyan denote the (controlled) offense players, Red denotes the (uncontrolled) defense player and goal keeper, and Purple denotes the ball. In both cases, our model improves the result -- in (a), while Agent2D kicks the ball towards the goalkeeper, our model aims toward the free side of the goal (b). In (c), Agent2D runs out of time to score, while our model predicts a more efficient trajectory (d). 
    % Note that even though our predictions for the ball are somewhat jagged, it still remains close to the distribution of the data and does not diverge too far from its realistic path. 
    }
    \label{fig:hfo_traj_opt}
    \vspace{-1em}
\end{figure}

\subsubsection{Safe Zone Predator-Prey}
% Using the same trained model\footnote{This also shows the power of model-based RL: without re-training the model, the agent optimizes for a new task successfully having never seen it before.}, we modified the task of the predator-prey environment by changing the cost function. 
In this scenario, there exists an area where the predator incurs no reward for being near the prey, and the prey is not penalized for the predator being close to it. This scenario is ideal for conducting CVaR optimization, the results of which we show in fig.~\ref{fig:fc_cvar}. Comparing the various cases, it is clear that risk-averse or risk-seeking optimization leads to either competitive or cooperative behavior, respectively. 

% OK: Consider removing both this and the table it refers to. Results are not as "impressive" as the other table, and are clearer in the visual figure. Might be a good space saver...
In addition to the visual results in fig.~\ref{fig:fc_cvar}, we tested the model over 100 episodes with random starting locations for predator and prey, with the predator using the learned TSM, and the prey escaping using a worst-case selection from the exploration policy. Table~\ref{tab:fc_cvar} compares the results of trajectory optimization when optimizing for the risk-averse (worst case) and the neutral (average) behavior of the prey. The results show clearly that using a risk-averse optimization scheme fares better against an adversarial opponent.



\subsection{RoboCup 2D Simulation}\label{sec:hfo}

RoboCup \cite{kitano1997robocup} is a well-known and diverse robotic soccer domain, which poses a challenge for many fields of research, from robotics to RL. The RoboCup 2D Soccer Simulation is a subdomain of RoboCup which focuses on agent strategy and cooperation. We use the Half Field Offense (HFO) environment \cite{kalyanakrishnan2006half,barrett2017making}, which is based on RoboCup 2D Simulation, to test our method in a challenging multi-agent environment. The scenario we play is a 2 vs. 2 game, where two offensive agents holding the ball attempt to score against a defender and a goalkeeper. The game ends when either a goal is scored, the defense touches the ball, the ball goes out of bounds or a certain time limit is reached. 

The exploration policy we use to collect data for the HFO domain is a hand coded one, native to the RoboCup simulator, named Agent2D. 
% Agent2D uses heuristics of distances between agents and open angles towards the goal to decide when to dribble the ball, pass it to other players or shoot it. 
We collected 17k trajectories of Agent2D agents playing against each other, where the observation space includes the locations and velocities of all agents and the ball, as well as player distance from the ball. 

Using this data, we trained TSMs for the various agents (see implementation details in the supplemental material). Rather than creating a model for each player separately, we consider the offense agents as one player ($x$) and the defense players as the adversary ($y$). Looking at both offensive players as a single agent allows us to plan a strategy for the entire offense, and does not limit us to the local actions of each player. The model for the offensive agent predicts the dynamics of the whole game, while the adversarial model is conditioned on the offense segment, following the conditional setting described in Sec.~\ref{sec:cond_msgm}. 
% An additional feature of the HFO domain is the ball, which does not select its own actions but responds to the actions of both offense and defense players. To model its behavior, we use a deterministic architecture based on the TSM decoder. 

Using the models learned from this dataset, we perform trajectory optimization for the task of scoring a goal. We incur a cost of 0 when a goal is scored and 1 for each time step without a goal. 
% This formulation not only promotes goal scoring, but also pushes the agent to score sooner in the game.
Using trajectories optimized for this task, our models predict scoring in scenarios where the Agent2D policy fails to do so (starting from the same initial positions). Due to technical difficulties with the HFO domain (such as inaccurate state information) we were not able to execute predicted trajectories in the simulator. Therefore, our results are qualitative examples (in fig.~\ref{fig:hfo_traj_opt} and the supplementary material) demonstrating multi-agent optimization. 

An additional observation arising from the HFO experiments is that the resulting latent space does indeed encode a strategy space, as different areas in the latent space correspond to different offensive strategies -- see fig.~\ref{fig:hfo_strategies} and the supplementary material for examples. 
% We leave further exploration of the structure of the latent space for future work. 

\section{Conclusion}
% TODO: the conclusion is going to be different from the one in the AAAI submission; needs rewriting

% TSMs are a promising approach to model based RL, which circumvent challenges like the accumulation of error when rolling out model predictions, and the tendency of the optimization to exploit errors in the model. 
In this work, we extended the idea of multi-step generative models to handle multi-agent problems, building on risk-sensitive optimization and sampling. We have applied our two suggested methods, of disentangled mutual information models and conditional models, to two domains, a predator-prey game (with several sub-tasks) and a simulated RoboCup environment. Our results show that the multi-agent TSM models effectively capture a reasonable `strategy space' of the agents, and that optimization in this space leads to realistic plans for execution. This results in an effective and interpretable decision making algorithm.

% In future work, we will explore how to apply these ideas to domains with a large number of agents, and domains with more complex observation structure such as images.


\bibliography{references.bib}
\bibliographystyle{icml2019}

%% Comment out when generating PDF for submission
\clearpage

\appendix
\section{Training Algorithm}
The following algorithm is the training flow for our models. $\texttt{Enc}$ and $\texttt{Dec}$ are the encoder and decoder of the Conditional Variational Autoencoder, and their architecture depends on the specific model (see below). When training the conditioned model (see Sec.~\ref{sec:cond_msgm}, the decoder is also conditioned on $y^+$ and $y^-$.
$\texttt{InfoEnc}$ are additional encoders arising from the mutual information lower bound described by \citet{chen2016infogan}: 
\begin{align*}
    \begin{split}
        L_I&(f, Q) = \\
        &\mathbb{E}_{Z_1\sim P(Z_1),X^+_1\sim f(Z, X^-)}[\log Q(Z_1|X_1^+)] + H(Z_1) \leq \\ 
        & I(Z_1, f(Z, X^-)) = I(Z_1, X^+_1)
    \end{split}
\end{align*}
We model $Q(Z_1|X^+_1)$ as an additional encoder, which attempts to reconstruct $Z_1$ from $\hat X^+_1$ mentioned above. Since the prior for $Z$ (and consequently, $Z_1$ and $Z_2$) is fixed, we can ignore it and only optimize for the expectation term, which can be interpreted as the negative MSE between $Z_1$ and $Q(Z_1|\hat X^+)$.
We used three weighting factors ($\gamma, \lambda_1, \lambda_2$) to weight the different parts of the loss function. We find that some hyper-parameter tuning on those coefficients is needed to receive working models. 
\begin{algorithm}
    \caption{Multi-Agent Multi-Step Generative Model Training}
    \label{alg1}
    \begin{algorithmic}[1]
        \STATE $\mathcal{D}\leftarrow \{(x^-,x^+)\}_{i=1}^N$ Initialize dataset with pairs of matching past and future segments
        \STATE $B, \texttt{Enc}, \texttt{Dec}, opt\leftarrow$ Initialize batch size, model (encoder and decoder) and optimizer
        \STATE $\gamma, \lambda_1, \lambda_2 \leftarrow $ Initialize loss weighting parameters
        \IF {Disentangled model}
            \STATE $\texttt{InfoEnc}_{1,2} \leftarrow $ Initialize encoders for mutual information maximization
        \ENDIF
        \FORALL{epochs}
            \FORALL{samples of $B$ pairs in  $\mathcal{D}$}
                \STATE $\mu_z, \sigma_z = \texttt{Enc}(x^+)$
                \STATE Sample $\{z\}_1^B \sim N(0, I)$
                \STATE $\hat x^+ = \texttt{Dec}(x^-, z \cdot \sigma_z + \mu_z)$
                \STATE $\ell = \text{MSE}(\hat x^+, x^+) - \gamma \mathcal{D}_{KL}[\mathcal{N}(\mu_z, \sigma_z)||\mathcal{N}(0,I)]$ 
                \IF {Disentangled model}
                    \STATE $\ell \leftarrow \ell - \lambda_1 \text{MSE}(\texttt{InfoEnc}_1(x^+_{(1)}, z_{(1)}) - \lambda_2 \text{MSE}(\texttt{InfoEnc}_2(x^+_{(2)}, z_{(2)})$
                \ENDIF
                \STATE Backprop$(\ell)$
                \STATE opt.step()
            \ENDFOR
        \ENDFOR
        \STATE Return trained model
    \end{algorithmic}
\end{algorithm}

\section{Trajectory Optimization Algorithm}
We provide pseudo-code for our method. This version shows the optimization when using the conditional model (Sec.~\ref{sec:cond_msgm}), however, it can be easily modified for the disentangled model version (Sec.~\ref{sec:disentangled}) by replacing lines 11-12 with a draw from a single shared model.

\begin{algorithm}
    \caption{Multi-Agent Trajectory Optimization}
    \label{alg2}
    \begin{algorithmic}[1]
        \STATE $x_0, y_0\leftarrow $ Initialize agents' states
        \STATE $N, m, l, k \leftarrow$ initialize batch size (number of optimization restarts), non-controllable agent trajectory samples, latent dimension of $Z$, segments per game
        \STATE $a = \alpha m$ risk sensitivity
        % \FORALL{$i$ in game segments (MPC loop)} 
          \STATE $z \leftarrow$ initialize latent variable $(n \times k \times l )$ by sampling from $\mathcal{P}_{prior}(Z)$
          \STATE $w \leftarrow$ sample latent variable $(m \times k \times l )$ from $\mathcal{P}_{prior}(W)$
          \STATE opt $\leftarrow$ initialize  optimizer (Adam)
          \FORALL{restarts $i$ in $n$}
            \FORALL{epochs}
                \FORALL{samples $j$ in $m$}
                    \FORALL{game segments}
                        \STATE $x^+_{i,j} = f^x(x^-_{i,j}, y^-_{i,j}, z_i)$
                        \STATE $y^+_{i,j} = f^y(x^-_{i,j}, y^-_{i,j}, x^+_{i,j}; w_j)$
                    \ENDFOR
                    \STATE loss$_{i,j} = -r_x(x_{i,j}$, $y_{i,j})$ summed over all segments
                \ENDFOR
                \STATE Sort loss$_{i,j}$ in increasing order along $j$
                \STATE loss$_{i} = \frac{1}{a}\sum_{j=1}^{a} \text{loss}_{i,j}$
            \ENDFOR
            \STATE Backprop loss
            \STATE opt.step()
        % \ENDFOR
        \ENDFOR
        \STATE Return trajectory $x_{i,j}$ that corresponds to the lowest $i$ in loss$_{i}$ and the highest $j$ in loss$_{i,j}$
    \end{algorithmic}
\end{algorithm}

\section{Predictions from the Disentangled Model}
To ensure that our disentangled setting of the model learns representations where different parts of the latent space control different parts of the output (i.e. different players), we run a simple experiment: we set one part of the latent space ($z_1$) to a constant value, and sample from the prior distribution to obtain values for the other part ($z_2$). We then use this latent variable construct, along with past segments, to predict future segments using our decoder. We expect to produce trajectories where one agent acts in a deterministic manner (as given $Z$, $D(X^-, Z)$ is a deterministic function) and the other agent producing a distribution over possible trajectories. Fig.~\ref{fig:freeze} shows example results of this experiment. 

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{info_sep1.png}
        \label{fig:freeze1}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{info_sep2.png}
        \label{fig:freeze2}
    \end{subfigure}
    \caption{Two examples of the bumper box domain, sampled from the disentangled model with one part of the latent space 'frozen' (set to a constant value), and the other part sampled from the prior. As expected, the behavior displayed is deterministic for one player, and distributed for the other. Red marks the distributed predictions for one agent, caused by sampling its latent variable from the prior. Blue trajectories are the ones predicted when the latent variable is 'frozen', thus causing deterministic behavior. Magenta and cyan lines denote the original trajectories collected from data, for reference. } \label{fig:freeze}
    % \vspace{-3em}
\end{figure}

\section{Detailed Implementation Parameters for Bumper Box}
Data for the bumepr domain was collected using the exploration policy described in \ref{sec:particle}, modified such that the random direction selection is weighted towards the location of the other agent to promote collisions between the agents, which are an area of interest in the state space. The observation for each agent is the location and velocity of both itself and its counterpart.
Similarly to \citet{mishra2017prediction}, we used an encoder with two layers of dilated causal convolutions and Tanh activations, and a decoder with three dilated causal convolution layers and an additional 1-dimensional convolution at the output. The decoder activation functions are the same as suggested for this type of architecture \cite{van2016wavenet} and used by \citet{mishra2017prediction}:
\begin{align}
\tanh(W_{f,k} * s + V^T_{f,k}z) \odot \sigma(W_{g,k} * s + V^T_{g,k}z)
\end{align}
where $*$ denotes a convolution, $\odot$ is element-wise multiplication, $s$ is the output of the previous layer, $z$ is the latent variable and both $V$ and $W$ are learned weights. For the disentangled model (Sec.~\ref{sec:disentangled}), we added two additional encoder networks to enable mutual information maximization between parts of the latent space and corresponding parts of the output. 
We found that a segment length of 10 steps and latent spaces of dimension 8 or 12 were a good choice for accurately learning the environment dynamics. We trained our model with Adam for 2000 epochs, using the standard hyper-parameters.  

\section{Detailed Implementation Parameters for Predator Prey}
In this domain, we used a slightly different observation space, reflecting the fact that agents rarely interact and are dependent only in their reward. Each agent's observation space included its location, its velocity and a vector pointing to the middle of the obstacle. During training, we offset the agent location (but not the obstacle vector) by the first location in the segment. In this manner, we trained the same models for both predator and prey agents. 
Similarly to the bumper box domain, we used an 8-dimensional latent space and 10-step segments. As this domain is somewhat less complicated, training tended to converge faster (even though we used somewhat smaller batch sizes). All other architecture parameters were the same as described in the previous section. 
As described in Sec.~\ref{sec:pred_prey}, we also trained a single-step baseline for this scenario. After conducting an architecture search, we concluded that a fully-connected, 3-layer MLP performed as well as any of the other architectures, and used it as a baseline for its simplicity of implementation. 

\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.22\textwidth}
        \includegraphics[width=\textwidth]{strat12.png}
        \caption{Single player, left}
        \label{fig:strat_alone_top}
    \end{subfigure} \hspace{0.02\textwidth}
    \begin{subfigure}[b]{0.22\textwidth}
        \includegraphics[width=\textwidth]{strat14.png}
        \caption{Single player, right}
        \label{fig:strat_alone_mid}
    \end{subfigure} \hspace{0.02\textwidth}
        \begin{subfigure}[b]{0.22\textwidth}
        \includegraphics[width=\textwidth]{strat15.png}
        \caption{One pass}
        \label{fig:strat_pass_once}
    \end{subfigure} \hspace{0.02\textwidth}
    \begin{subfigure}[b]{0.22\textwidth}
        \includegraphics[width=\textwidth]{strat11.png}
        \caption{Two passes}
        \label{fig:strat_pass_twice}
    \end{subfigure}
    % \framebox[\columnwidth]{\rule{0pt}{160pt}}
    \caption{Plots of the trajectories predicted for four random latent variable draws. Blue and cyan lines are the two offense players (controlled by the agent) and red lines denote the defense players. The purple line denotes the ball. Trajectories are divided into segments of 10 time steps, and circles indicate the segment index. In~\ref{fig:strat_alone_top} the agent plans a strategy where the blue player advances alone and shoots the ball from the left. In~\ref{fig:strat_alone_mid} a different strategy arises, with the blue player dribbling the ball towards the right of the field and kicking from there. In~\ref{fig:strat_pass_once} the strategy is yet again different, and incorporates blue catching the ball and passing it to cyan, who in turn shoots. \ref{fig:strat_pass_twice} shows an altogether different strategy, in which the cyan player catches the ball and passes it to blue. }
    \label{fig:more_strategies}
\end{figure*}

\section{Detailed Implementation Parameters for HFO 2 vs. 2}
 As in the Multi-Agent Particle Environment, we found an 8-dimensional latent space and a 10-step segment were suitable to capture the dynamics. We also used a similar architecture to the one described above. However, we found we needed our models to be somewhat more expressive, and added channels to each convolution. Moreover, instead of predicting the next agent location directly, the models we trained for this domain predict the change in location and velocity, and add it to the previous known location to create future states. 
 Finally, for ease of training, we equalized the length of all collected data trajectories to 100 time steps, truncating longer ones and repeating the final state of shorter ones. This enables us to train without some sort of 'end scenario' signal.
 
 \section{Additional examples for Strategy Space Planning in HFO}
 As described in Sec.~\ref{sec:hfo} and demonstrated in Fig.~\ref{fig:hfo_strategies}, drawing different samples from the latent space can provide completely different \emph{strategies} for the offensive agents, and does not just affect the trajectory details. This can be clearly seen in fig.~\ref{fig:more_strategies}, in which each trajectory is the (non-optimized) result of different samples of the latent space, all from the same starting location. 

\end{document}


==> main_neurips.tex <==
% \documentclass{article}

% if you need to pass options to natbib, use, e.g.:
%     \PassOptionsToPackage{numbers, compress}{natbib}
% before loading neurips_2019

% ready for submission
% \usepackage{neurips_2019}

% to compile a preprint version, e.g., for submission to arXiv, add add the
% [preprint] option:
%     \usepackage[preprint]{neurips_2019}

% to compile a camera-ready version, add the [final] option, e.g.:
    %  \usepackage[final]{neurips_2019}
     \usepackage{neurips_2019}

% to avoid loading the natbib package, add option nonatbib:
%     \usepackage[nonatbib]{neurips_2019}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography

% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{color}
\usepackage{subcaption}
\usepackage{booktabs} % for professional tables

\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{tabularx}
\usepackage{algorithm}
\usepackage{algorithmic}

%%% Comments
\newcommand{\mycomm}[3]{{\color{#2} \textbf{[#1: #3]}}} 
%define your comment NAME and COLOR here
\newcommand{\AT}[1]{\mycomm{AT}{magenta}{#1}}
\newcommand{\OK}[1]{\mycomm{OK}{cyan}{#1}}


\title{Multi Agent Reinforcement Learning with Multi-Step Generative Models}

% The \author macro works with any number of authors. There are two commands
% used to separate the names and addresses of multiple authors: \And and \AND.
%
% Using \And between authors leaves it to LaTeX to determine where to break the
% lines. Using \AND forces a line break at that point. So, if LaTeX puts 3 of 4
% authors names on the first line, and the last on the second line, try using
% \AND instead of \And before the third author name.

\author{%
  Orr Krupnik \\
  Technion - IIT \\
  Haifa, Israel \\
  \texttt{ok1@campus.technion.ac.il} \\
  % examples of more authors
   \And
   Igor Mordatch \\
   OpenAI \\
  % Address \\
  % \texttt{email} \\
   \And
   Aviv Tamar \\
   Technion - IIT \\
   Haifa, Israel \\
   \texttt{avivt@technion.ac.il} \\
  % \And
  % Coauthor \\
  % Affiliation \\
  % Address \\
  % \texttt{email} \\
}

\begin{document}

\maketitle 

\begin{abstract}
The dynamics between agents and the environment are an important component of multi-agent Reinforcement Learning (RL), and learning them provides a basis for decision making. However, a major challenge in optimizing a learned dynamics model is the accumulation of error when predicting multiple steps into the future. 
Recent advances in variational inference provide model based solutions that predict complete trajectory segments, and optimize over a latent representation of trajectories. For single-agent scenarios, several recent studies have explored this idea, and showed its benefits over conventional methods. In this work, we extend this approach to the multi-agent case, and effectively optimize over a latent space that encodes \emph{multi-agent strategies}. We discuss the challenges in optimizing over a latent variable model for multiple agents, both in the optimization algorithm and in the model representation, and propose a method for both cooperative and competitive settings based on risk-sensitive optimization. We evaluate our method on tasks in the multi-agent particle environment and on a simulated RoboCup domain.
\end{abstract}

\section{Introduction}
Many real world problems where multiple agents operate in the same environment can be cast as multi-agent systems. Examples include autonomous vehicles \citep{lee2017desire,chen2017socially,schmerling2017multimodal}, navigation in environments with humans \citep{ivanovic2018generative}, learning communication between agents \citep{mordatch2017emergence}, and multiplayer games \citep{stone2000layered,silver2016mastering}. 

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.22\textwidth}
        \includegraphics[width=\textwidth]{strat12.png}
        \caption{Single player offense}
        \label{fig:strat_alone}
    \end{subfigure} \hspace{0.02\textwidth}
    \begin{subfigure}[b]{0.22\textwidth}
        \includegraphics[width=\textwidth]{strat15.png}
        \caption{Passing players}
        \label{fig:strat_pass}
    \end{subfigure}
    % \framebox[\columnwidth]{\rule{0pt}{160pt}}
    \caption{Learning trajectory representations at the strategy level. We plot the trajectories predicted for two random latent variable draws in the RoboCup domain. Blue and cyan lines denote the two offense players (controlled by the agent) and red lines denote the defense players. The purple line denotes the ball. Trajectories are divided into segments of 10 time steps, and circles indicate segment starting points. In~(a) the agent plans a strategy where the blue player advances alone and shoots the ball from the left. In~(b) the strategy is different, and incorporates blue catching the ball and passing it to cyan. }
    \label{fig:hfo_strategies}
\end{figure}

In recent years, following advances in deep learning and reinforcement learning (RL) in particular \citep{sutton1998reinforcement}, there have been many attempts to apply RL to multi-agent domains. 
Research in RL can be classified into two main approaches: model-free RL and model-based RL. In model-free RL, agents attempt to learn a policy -- a mapping directly from states to actions, tuned to solve a specific task \citep{sutton1998reinforcement}. In model-based RL, learning techniques are applied to model the dynamics governing the environment. The learned model is then used for planning, enabling control in tasks for which agents were not specifically trained. In addition, model-based approaches are generally more sample efficient, thus converging faster and saving time when training RL agents in complex environments \citep{deisenroth2011pilco,kurutach2018model}. Finally, model-based methods are interpretable -- it is relatively easy to roll out a trajectory using a learned model, and analyze the knowledge encoded in it. In light of these benefits, this work focuses on model-based RL.

The application of model-based RL to complex, multi-agent domains presents significant challenges. 
% A major one lies in the way the model is learned. 
The typical approach for model learning involves predicting a single next state conditioned on past states and actions \citep{abbeel2005learning}. This method has some significant drawbacks, such as tending to accumulate error when rolled out multiple time steps into the future. 
% This typically occurs from accumulation of small errors at each step, or divergence from the distribution of states and actions explored during training, for example, when a collision occurs in a robotic domain \citep{mishra2017prediction}. 
When the dynamics are stochastic or the observation is noisy, both in single agent and multi-agent environments, this problem amplifies.

While multi-agent RL is difficult, game theory provides many guaranteed ways to solve multi-agent problems~\citep{cesa2006prediction}, but has mostly been studied in a `strategy space' formulation, where single actions are played against other agents, e.g. in matrix games. The aim of our work is to combine such strategic decision making into high-fidelity problems that can be captured by RL formulations, such as continuous control domains.

%%AT: here we need a paragraph about trajectory prediction models. 
For single-agent model-based RL, several recent studies proposed to mitigate the error accumulation problem by learning deep generative models of multi-step trajectory segments~\citep{mishra2017prediction,ke2018modeling,hafner2018learning,rhinehart2018deep}. Here, we collectively refer to these methods as \emph{multi-step generative models}. The idea in these approaches is to learn a distribution of future trajectory segments in an unsupervised manner, using a deep generative model (e.g. a VAE, \citealt{kingma2013auto}), and perform planning by searching in the latent space of the model.
% use some form of variational inference \citep{kingma2013auto} to embed future segments of multiple time steps in a low-dimensional latent space. 
In essence, the latent space captures a compact `strategy space' of the agent, and it has been shown that optimization over this latent space is more effective than optimizing over single-step actions. 

% This potentially avoids the error accumulation of iteratively rolling out one-step predictions, and has been shown to be more effective than optimizing over single-step actions. 
% The latent space can capture a compact 'strategy space' of the agent, and it has been shown that optimization over this latent space is more effective than optimizing over single-step actions. 
% All the aforementioned works, however, address a relatively simple domain, with a single agent and very few environment elements. Therefore, they are not well suited to multi-agent scenarios. 

We propose to solve multi-agent problems more efficiently by extending multi-step generative models to domains with multiple agents. 
% cooperating or competing in various tasks. 
Our idea is that by training a generative model for predicting trajectories of several interacting agents, we can capture a lower dimensional, more generalized representation of the states and actions that are likely in the data, thus comprising a `strategy space' of agent interaction, which can then be optimized using game theoretic ideas. An illustrative example in the RoboCup domain~\citep{kitano1997robocup} is provided in Fig.~\ref{fig:hfo_strategies}: here, different values of the latent variables correspond to different offense strategies, and optimization can be performed in a high-level strategy space instead of using low-level actions. 

We present a practical algorithm for trajectory optimization of multiple agents based on risk-sensitive optimization, and discuss several approaches to modeling trajectories for multiple agents that comply with planning based on latent-space search. We show that our method can learn effective models for continuous multi-agent domains with complex dynamics, both in the multi-agent particle environment~\citep{lowe2017multi} and on a simulated RoboCup domain.

% We show that our method can learn effective models for continuous multi-agent domains with complex dynamics, both in the such as a simulated RoboCup domain.


% We present a practical algorithm for trajectory optimization of multiple agents based on risk-sensitive optimization, using multiple TSMs learned separately for different types of agents. We show that our method can learn effective models for continuous multi agent domains with complex dynamics, such as a simulated RoboCup domain.

% Additionally, while the models described above optimize over agent actions to select future segments, we propose to learn a model which ignores the actions and generates future segments of states directly from the latent space. This creates a more flexible and diverse world model, which in turn leads to a more diverse set of policies to optimize over, and finally better trajectories. 

% OK: The following two paragraphs are from the previous submission and probably don't fit in the new version 
% One approach which aims to tackle the problems with model-based RL described above is presented by \citet{mishra2017prediction}, where a Temporal Segment Model (TSM) was proposed. TSMs learn a model which embeds future segments of multiple states in a low-dimensional latent space using a conditional variational autoencoder \citep{kingma2013auto}. This potentially avoids the error accumulation of iteratively rolling out one-step prediction models. The latent space can capture a compact 'strategy space' of the agent, and it has been shown that optimization over this latent space is more effective than optimizing over single-step actions. \citet{mishra2017prediction} also proposed a deep generative model based on a WaveNet architecture \citep{van2016wavenet} designed for continuous control tasks. This approach has been shown to outperform the single-step baseline, as well as methods rolled out multiple timesteps into the future, and more sophisticated frameworks such as LSTMs. 


% The latent space provides us with a lower dimensional, more generalized representation of the states and actions that are likely in the data, thus comprising a 'strategy space' of the agents.

\section{Related Work}
Many approaches consider model-based RL in domains with complex, stochastic dynamics. Our work is inspired by the Temporal Segment Models (TSMs) developed by~\citet{mishra2017prediction} and more recent approaches~\citep{ke2018modeling,hafner2018learning} which use conditional variational autoencoder (CVAE) based dynamics models to predict multiple time steps into the future based on a previous segment of states and actions. The dynamics model is then used to optimize over agent trajectories for a specific task. A different approach is taken by  \citet{nagabandi2017neural}, who use neural network dynamics models, combined with Model Predictive Control (MPC) and model-free fine tuning to achieve effective control and stable gaits in the MuJoCo baseline environment. \citet{williams2017information} also use MPC to learn from a trained dynamics model, achieving high levels of performance on both simulated and actual hardware tasks. The models used, however, are single time-step, fully connected neural network models,
% \citet{deisenroth2011pilco} learn a Gaussian process dynamics model and exploit the learned uncertainty structure to mitigate the effect of error accumulation during planning. 
and all the approaches described above consider only a single agent. 

Recently, model based approaches have also been successfully used to \textit{predict} the behavior of multiple agents in both cooperative and competitive environments. Most of these owe their success to advances in deep variational inference \citep{kingma2013auto}. \citet{lee2017desire} predict vehicle trajectories in environments with multiple counterparts, such as other vehicles and pedestrians. \citet{ivanovic2018generative} and \citet{schmerling2017multimodal} use CVAEs to predict human behavior for human-robot interaction. \citet{zheng2016generating} use deep RNN models to recreate trajectories of a team of basketball players. They provide the interesting observation of interpreting a latent variable as a 'macro-goal', which controls the strategy of an agent for a given period of time. This is similar to our interpretation of the latent space as a 'strategy space' for the agent to optimize in. To the best of our knowledge, our attempt to use the deep generative model and the prediction of agent behavior to \emph{optimize} over trajectories for a given task in a multi-agent environment is, as of yet, a novel contribution. 

% Other methods for multi-agent RL follow a model-free approach. We include them here for completeness, however, we choose to focus on model-based methods in this work for their advantages described above.
% The 'Decentralized Actor, Centralized Critic' of \citet{lowe2017multi} has been highly successful in solving specific tasks in mixed cooperative and competitive environments, similar to the ones we examine in this work. \citet{yang2018mean} average over the effects surrounding entities have on the controlled agent in order to scale up Actor-Critic and Q-Learning algorithms to large numbers of agents. Recently, \citet{jaderberg2018human} trained multiple agents in a simulated Capture the Flag game, using population based learning.

\section{New Formulation}
\input{formulation.tex}

\section{Background}
Many dynamical systems can be described and analyzed as Markov Decision Processes (MDPs, \citealt{sutton1998reinforcement}). At each time step of an MDP, the system is in some state $x_t \in \mathcal{X}$ and agents can perform actions $u_t \in \mathcal{U}$, where $\mathcal{X}$ and $\mathcal{U}$ are the sets of all possible states and actions, respectively. The dynamics of the system are some function $f$ such that $x_{t+1} = f(x_t, u_t)$ (or some probability distribution $\mathcal{P}(x_{t+1} | x_t, u_t)$), governing the transitions from one state of the system to the next. Given a reward function $r(x)$, the typical goal is to maximize the expected sum of rewards $\mathbb{E}\left[\sum_{t=0}^T r(x_t)\right]$.\footnote{Other common criteria include discounted and episodic formulations~\citep{sutton1998reinforcement}. Our results can be easily extended to these cases.}

% In the RL setting, the dynamics are assumed to be unknown. Model-based RL approaches learn a model for the dynamics, and then solve for a policy which maximizes rewards. Since in an MDP each state is dependent only on the previous one, the traditional approach for modelling the dynamics of a system attempts to approximate the transition function $f$ (or probability $\mathcal{P}$) using some function approximator, such as a feed-forward neural network~\citep{hunt1992neural,depeweg2017learning}. 

\subsection{Multi-step Generative Models}
%TODO: Cite TSMs, PlaNet, R2P2 etc., explain the idea of predicting a segment instead of a single timestep to get more accurate trajectories. Discuss prediction using latent space, and maybe mention predicting states directly and not actions. 
% Also, make sure this isn't redundant of the realted work section. 
% Relevant pargraphs from the original "Temporal Segment Models" section copied below. 

The traditional approach for modelling dynamics attempts to approximate the transition function $f$~\citep{hunt1992neural,depeweg2017learning}. Multi-step generative models (such as \citealt{mishra2017prediction,rhinehart2018deep,ke2018modeling}) learn a more generalized form of the system dynamics. Consider segments (or "chunks") of $H$ past agent observations $X^-=\{x_{t-H+1},...,x_{t}\}$ and segments of future observations $X^+=\{x_{t+1},...,x_{t+H}\}$. Multi-step models learn a distribution $P(X^+|X^-)$ to predict the segment of future states based on past states, thus enabling consideration of delayed effects of previous actions and capturing longer temporal relations between states than a single-step model. 

In this work we focus on the Temporal Segment Models (TSMs) of \citet{mishra2017prediction}, but the ideas presented here can be generalized to other multi-step generative models. 
% Note that the original TSMs described by \citet{mishra2017prediction} condition the model on past and future actions, while \citet{ke2018modeling} and \citet{hafner2018learning} condition on segments of past actions. However, we choose to omit the actions here for simplicity and to match our modifications to the model, explained below. Although this approach poses a harder learning problem, compelling us to learn both the dynamics and the decision making processes of other agents, conditioning over states alone generalizes our model and renders it a simpler solution, relieving us of the need to provide precise actions for every agent in the system.
TSMs use a CVAE architecture~\citep{kingma2013auto}, where an encoder learns a distribution over a latent variable $Z$ conditioned on future observations: $\mathcal{Q}(Z|X^+)$, 
while a decoder reconstructs $X^+$: 
% conditioned on $X^-$ and a sample from the latent variable $Z$, 
$\hat X^+ = D(X^-,Z)$.
% , modelling the distribution $\mathcal{P}^{(x)}(X^+|X^-)$. 
The CVAE model encodes the input $X^+$ to obtain the parameters $\mu_Z, \sigma_Z$ of a Gaussian distribution for the latent variable. 
The optimization objective is then a variational lower bound of the data log likelihood~\citep{kingma2013auto}:
% , as described by eq.~\eqref{eq:elbo}:
\begin{equation}
    \begin{split}
    \mathcal{L} = \mathbb{E}_{Z\sim Q(Z|X^+)} &\left[\log P(X^+|X^-,Z)\right] - \\ &\mathcal{D}_{KL}\left[Q(Z|X^+)||P_{prior}(Z)\right],
    \end{split}
    \label{eq:elbo}
\end{equation}
where $P_{prior}(Z) = \mathcal{N}(0,I)$, and $P(X^+|X^-,Z) = \mathcal{N}(D(X^-,Z),I)$.
% where the prior is a normal distribution $P_{prior}(Z) = \mathcal{N}(0,I)$.
Each instance of the latent variable describes a segment of observations, and the decoder can be used as a generative stochastic dynamics model, to create future segments $\hat X^+$ using samples from the prior. 
% See figure~\ref{fig:arch_orig} for a general scheme of the model architecture.

% OK: The following is specific TSM, should probably move to our architecture section
% For the model to be able to capture temporal relations between observations, both encoder and decoder networks incorporate several layers of dilated causal convolutions, similar to the WaveNet architecture \citep{van2016wavenet} which has proven extremely successful in capturing temporal relations and generating future predictions of both audio and images. The dilation enables the network to capture a wider receptive field of observation history, using a relatively small number of layers. Being fully convolutional, the resulting CVAE is differentiable and can be trained with backpropagation, using the reparametrization trick described by \citet{kingma2013auto}. Networks based on dilated causal convolutions have recently been shown to train more efficiently than other sequential architectures, such as RNNs \citep{bai2018empirical}. 

One of the motivations for learning a dynamics model is to later use this model to solve the MDP problem. Assume that the total horizon of interest $T$ can be segmented to $k$ segments of length $H$. Then, the learned model for future segment distribution $\mathcal{P}^{(x)}(X^+|X^-,Z)$ can be rolled out $k$ times to produce a distribution for a $T$-length trajectory, which we denote as $\mathcal{P}^{(x)} (x_{t} \vert x_{0:t-1}, z^{(1:k)})$, where $z^{(1:k)}$ denotes $k$ samples of the latent variable $Z$.
\citet{mishra2017prediction} suggest the following trajectory optimization problem:\footnote{In the model of \citet{mishra2017prediction}, the latent space actually encoded an action distribution $\mathcal{P}^{(u)}(U^+|U^-,Z)$, and the optimization problem was of the form: 
$    \max_{z^{(1)},...,z^{(k)}} \mathbb{E} \left[ \sum_{t=1}^{T} r(x_{t},u_{t}) \right] \quad
    \textrm{s.t. } x_{t} \sim \mathcal{P}^{(x)} (x_{t} \vert x_{0:t-1}, u_t) ,
    u_{t} \sim \mathcal{P}^{(u)} (u_{t} \vert x_{0:t-1}, z^{(1:k)}).
$
Here, we present a similar optimization problem for a model that considers state trajectories without direct action encoding.
} 
\begin{equation}
    % \begin{split}
    \max_{z^{(1:k)}} \mathbb{E} \left[ \sum_{t=1}^{T} r(x_{t}) \right],\quad 
    \textrm{s.t. } x_{t} \sim \mathcal{P}^{(x)} (x_{t} \vert x_{0:t-1}, z^{(1:k)}).
    % \end{split}
    \label{eq:traj_opt_clean}
\end{equation}
Note that the optimization is over the latent space $Z$ -- the latent space of the agent trajectory. In this sense, we are optimizing over the possible strategies that the agent can perform, as displayed in the data used for training the model. Problem \eqref{eq:traj_opt_clean} can be solved using gradient descent.\footnote{The distribution $\mathcal{P}^{(x)}(X^+|X^-,Z)$ is typically represented as a neural network that encodes the mean of a Gaussian. Then, the expectation in \eqref{eq:traj_opt_clean} can be approximated with the deterministic prediction of the mean trajectory.}


\section{Multi-Agent Multi-Step Generative Models}
In this paper, we consider an extension to the MDP model for a multi-agent setting known as a Markov Game~\citep{littman2001value}. For simplicity, we present the case of two agents, but our results can easily be extended to more players (e.g. as described by \citealt{littman2001value}). 
Consider two agents $x$ and $y$ acting in a dynamic environment. At time-step $t$, the states of the agents are denoted by $x_t$ and $y_t$, respectively. The agents each select an action $a_t \in \mathcal{A}$ and $b_t \in \mathcal{B}$, out of their respective action sets. The dynamics of the environment are then governed by the distribution (or function) $\mathcal{P}(x_{t+1}, y_{t+1} \vert x_t, y_t, a_t, b_t)$, and the agents obtain rewards $r_x(x_t,y_t)$ and $r_y(x_t,y_t)$, respectively. This formulation can be used to define adversarial scenarios (e.g. by selecting zero sum rewards), cooperative scenarios (e.g. by selecting the same reward function for both agents), or various combinations thereof. To simplify our presentation, in this work we focus on the case of deterministic dynamics, given by $x_{t+1}, y_{t+1} = f(x_t, y_t, a_t, b_t)$.\footnote{An extension to stochastic dynamics can be done by adding another uncontrolled agent with action $c$ that represents noise, and writing the transition as $x_{t+1}, y_{t+1} = f(x_t, y_t, a_t, b_t, c_t)$. We leave a full investigation of stochastic dynamics to future work.}

In our setting, we consider a case where only agent $x$ is controlled, while the policy and reward driving agent $y$ are not known. In particular, we do not assume that $y$ has any fixed behavior. Our goal is to optimize the sum of rewards for agent $x$ in this case. In the remainder of this section, we first describe our optimization criterion, and later discuss how to learn suitable generative multi-step models in order to optimize it.

\subsection{Risk-Sensitive Optimization Formulation}\label{sec:risk}
To solve the multi-agent decision problem above, we propose to learn a probabilistic model for the \emph{possible} behaviors of $y$, 
% $\mathcal{P}(b|x,y)$, 
as seen in the data, and optimize a \emph{risk-sensitive} behavior policy for $x$, where the risk attitude would correspond to our belief about the nature of agent $y$'s policy. In particular, we consider the conditional value at risk measure (CVaR, a.k.a.~expected shortfall, \citealt{rockafellar2000optimization}). The CVaR at level $\alpha$\% of a random variable denotes the expectation of the variable on the worst (or best) $\alpha$\% of cases. Intuitively, as we optimize for the worst (best) cases, we take into consideration the adversarial (cooperative) nature of the other agents in the game. This statement has been made concrete by \citet{artzner1999coherent}. In this work, therefore, we opt to maximize the risk-averse CVaR of agent $x$'s sum of rewards:  $\mathbb{E}\left[\left.\sum_{t=0}^T r(x_t,y_t)\right|\sum_{t=0}^T r(x_t,y_t) \leq Q_\alpha\right]$, where $Q_\alpha$ denotes the $\alpha$-quantile of the sum of rewards, and the expectation is taken with respect to agent $y$'s behavior. 
% $\mathcal{P}(b|x,y)$. 
Note that when $\alpha=1$, we obtain the expected sum of rewards, while for $\alpha \to 0$ we optimize for the worst case. \footnote{To maximize a risk-seeking agent, we consider  $\mathbb{E}\left[\left.\sum_{t=0}^T r(x_t,y_t)\right|\sum_{t=0}^T r(x_t,y_t) \geq Q_\alpha\right]$. In this case, $\alpha=0$ corresponds to the expected sum of rewards, while for $\alpha \to 1$ we optimize for the best case.}

Solving the risk-averse optimization problem would correspond to planning for an adversarial $y$, while computing a risk-seeking behavior would correspond to the assumption that $y$ is cooperative. Solving for the expectation, in this case, would be a 'middle ground' between assuming that $y$ is adversarial or cooperative. We next discuss how to learn suitable models for the behavior of $y$.

\subsection{Multi-Agent Temporal Segment Models}\label{sec:matsm}
In the following, we extend the TSM (and general multi-step generative models) to the Markov game setting. 

As discussed above, for the risk-sensitive optimization criterion (and also for other traditional game theoretic formulations, \citealt{cesa2006prediction}) we require a model for the possible behaviors of $y$. For a single-step dynamics model, it is easy to learn the distribution of $y$'s actions from data. Recall, however, that the main motivation behind multi-step generative models is to eliminate the need to model the effect of single actions on the state, and instead model state trajectory segments for both agents.
% How then, could we learn a multi-step generative model that is compatible with the CVaR optimization criterion?

We begin with an important observation: in the standard TSM and MDP setting, we can interpret the latent variable $Z$ as a code for the sequence of actions in a segment $\{u_{t},...,u_{t+H-1}\}$. The reason is that any feasible trajectory $\{x_{t+1},...,x_{t+H}\}$ in the system can be realized by some sequence of actions, so a distribution on the trajectories can be represented by a distribution on the actions that induce them (as it is just a change of variables). 

To simplify notation, we restrict our presentation to optimizing a single segment. The extension to a full trajectory is done by rolling out several segments, as in Eq.~\ref{eq:traj_opt_clean}. Similarly to the definitions of $X^-$ and $X^+$, let $Y^-$ and $Y^+$ denote the segments of $H$ past and future observations for agent $y$. For a two player game, we would like to learn a generative model for the distribution $P(X^+,Y^+|X^-,Y^-)$ with two latent components, $Z$ and $W$, which correspond to the sequences of actions in a segment for agent $x$, $\{a_{t},...,a_{t+H-1}\}$, and agent $y$, $\{b_{t},...,b_{t+H-1}\}$, respectively. Such a representation would allow us to cast the trajectory optimization problem in a standard game theoretic formulation, where the spaces of $Z$ and $W$ denote the possible strategies for each agent. For the CVaR objective, we would have:
\begin{align}
    \begin{split}
    \max_{z} & \textrm{ CVaR} \left[ \sum_{t=1}^{H} r(x_{t},y_{t}) \right] \\
    \textrm{s.t. } &x_{t},y_{t} \sim P(X^+,Y^+|X^-,Y^-, z, w), \\
    & w \sim P_{prior}(W).
    \end{split}
    \label{eq:traj_opt_multi}
\end{align}
However, learning such a generative model is not trivial, since the contribution of each action sequence to agent trajectories in the segment depends also on the dynamical system $f$, which is not known in advance. In the rest of this section, we propose two approaches for overcoming this problem. The first is by learning disentangled latent representations, and the second is by learning conditional models, which we show are sufficient under certain assumptions.  

\subsubsection{Disentangled Multi-Step Generative Models} \label{sec:disentangled}
Latent spaces in multi-step generative models are generally unstructured \citep{mishra2017prediction,rhinehart2018deep}, and cannot be queried to control various aspects of the predicted segment. Here, we propose a representation where the elements of the latent space are \emph{disentangled} with respect to their effect on the two agents' strategies. That is, some elements in the latent space control the strategy of agent $x$, while other elements control the strategy of $y$.
% Such a "seperability" property would be extremely helpful when optimizing models for multiple agents, as each part of the latent space could be trained to control the future trajectories of different agents. 
% We borrow ideas from \citet{chen2016infogan} and \citep{klys2018learning}, where the latent spaces of generative models are partitioned to control various aspects of the generated output. 

To learn such a representation, we borrow ideas from \citet{chen2016infogan} and \citet{klys2018learning}, and propose to use the notion of mutual information to induce dependency between elements in the latent space and desired elements in the predicted trajectory. 

The mutual information between random variables $Q$ and $V$ is:
% \begin{equation*}
$
    I(Q;V) = H(Q) - H(Q|V) = H(V) - H(V|Q),
$
% \end{equation*}
where $H(Q)$ denotes the entropy of $Q$, and $H(Q|V)$ denotes the conditional entropy~\citep{cover2012elements}. Following the discussion above, to induce a disentangled latent representation for $X$ and $Y$ we would like to maximize the mutual information between $Z$ and $X$, and between $W$ and $Y$. We therefore propose the following loss function for training the generative model:
\begin{equation}\label{eq:loss_info}
    \min_\theta \mathcal{L} - \lambda_1 I(Z; X^+) - \lambda_2 I(W; Y^+)
\end{equation}
where $\mathcal{L} = \mathbb{E}_{Z,W\sim Q} \left[\log P(X^+,Y^+|X^-,Y^-,Z,W)\right] - \mathcal{D}_{KL}\left[Q(Z,W|X^+,Y^+)||P_{prior}(Z,W)\right]$ is the evidence lower bound~\citep{kingma2013auto}, and $\lambda_1>0$ and $\lambda_2>0$ are weights on the mutual information terms. To optimize \eqref{eq:loss_info} in practice, we use the lower bound proposed by \citet{chen2016infogan} We provide a full algorithm (Alg.~\ref{alg1}) in the supplementary material.
% and a part of the output future prediction, $X^+_1$ (completing the notation from the previous subsection). 
% Therefore, incorporating our variational lower bound from eq.~\eqref{eq:elbo}, the optimization objective of learning our model becomes: 
% \begin{align}
%     \min_\theta \mathcal{L} - \lambda I(Z_1, X^+_1) 
% \end{align}
% As noted by \citet{chen2016infogan}, in practice, maximizing the mutual information term directly is hard, since it requires access to the posterior $\mathcal{P}(Z|X^+)$. We can instead lower bound the information term using Variational Information Maximization \citep{agakov2004algorithm}. As shown by \citet{chen2016infogan}, the lower bound can be written as:
% \begin{align}
%     \begin{split}
%         L_I(f, Q) &= \mathbb{E}_{Z_1\sim P(Z_1),X^+_1\sim f(Z, X^-)}[\log Q(Z_1|X^+)] + H(Z_1) \leq \\ 
%         &\leq I(Z_1, f(Z, X^-)) = I(Z_1, X^+_1)  = H(z_1) - H(Z_1|f(Z, X^-))        
%     \end{split}
% \end{align}

\subsubsection{Conditional Multi-Step Generative Models} \label{sec:cond_msgm}
An alternative disentangled model representation can be obtained by conditioning. Since $P(X^+,Y^+|X^-,Y^-)=P(X^+|X^-,Y^-)P(Y^+|X^-,Y^-,X^+)$, we can learn two independent models: one for $P(X^+|X^-,Y^-)$ with a latent variable $Z$, and one for $P(Y^+|X^-,Y^-,X^+)$ with a latent variable $W$. Such will guarantee that the latent variables $Z$ and $W$ represent the strategies of $X$ and $Y$, respectively. However, such a formulation is not necessarily compatible with our CVaR optimization approach.

Since we are optimizing over $Z$, and $P(X^+|X^-,Y^-)$ does not depend on the value of $W$, we are effectively letting agent $x$ `play first', and choose its trajectory, while agent $y$ can only react to the trajectory of $x$ that has already been chosen.\footnote{Conversely, if we model the distribution as $P(Y^+|X^-,Y^-)P(X^+|X^-,Y^-,Y^+)$, we are giving an advantage to player $y$.} This gives a clear advantage to player $x$, which we demonstrate in our experiments in a scenario where players can block each other (see fig.~\ref{fig:bumpers}). 

However, the conditional representation is still appropriate under some conditions. Consider a system where the dynamics of the agents are independent, i.e., can be written as $x_{t+1} = f_x(x_t, a_t)$ and $y_{t+1} = f_y(y_t, b_t)$, while the coupling between the agents is realized only through the reward function $r(x,y)$. In such cases, learning two independent models for the agents is compatible with the CVaR optimization. While this representation is limited in its applicability, its simplicity is an advantage in practice and, as we show in our experiments, it is suitable for several interesting domains such as the RoboCup simulation.

% The below is math we wrote a few months ago, which may describe the model a little better than the paragraph below it (of course we'll still need the CVaR parts)
% Is the conditional model always enough? Can we think of a scenario where we need a shared model for different agents? \\
% $P(x,y) = P(x|y)P(y)$ \\

% \subsection{Information Theoretic Generative Models}
% Latent spaces in multi-step generative models are generally unstructured \citep{mishra2017prediction,rhinehart2018deep}, and cannot be queried to control various aspects of the predicted segment. Such a "seperability" property would be extremely helpful when optimizing models for multiple agents, as each part of the latent space could be trained to control the future trajectories of different agents. We borrow ideas from \citet{chen2016infogan} and \citep{klys2018learning}, where the latent spaces of generative models are partitioned to control various aspects of the generated output. 

% We propose to use the notion of mutual information \eqref{eq:mut_inf} to enforce a relation between parts of the latent space and parts of the output variable. A general definition of mutual information is given by: 
% \begin{align}
%     I(X;Y) = H(x) - H(X|Y) = H(Y) - H(Y|X)
% \end{align}
% Where $H(X)$ denotes the entropy of a random variable $X$, and $H(X|Y)$ denotes the conditional information. In our case, we'd like to maximize mutual information between a part of the latent space, denoted by $Z_1$, and a part of the output future prediction, $X^+_1$ (completing the notation from the previous subsection). Therefore, incorporating our variational lower bound from eq.~\eqref{eq:elbo}, the optimization objective of learning our model becomes: 
% \begin{align}
%     \min_\theta \mathcal{L} - \lambda I(Z_1, X^+_1) 
% \end{align}
% As noted by \citet{chen2016infogan}, in practice, maximizing the mutual information term directly is hard, since it requires access to the posterior $\mathcal{P}(Z|X^+)$. We can instead lower bound the information term using Variational Information Maximization \citep{agakov2004algorithm}. As shown by \citet{chen2016infogan}, the lower bound can be written as:
% \begin{align}
%     \begin{split}
%         L_I(f, Q) &= \mathbb{E}_{Z_1\sim P(Z_1),X^+_1\sim f(Z, X^-)}[\log Q(Z_1|X^+)] + H(Z_1) \leq \\ 
%         &\leq I(Z_1, f(Z, X^-)) = I(Z_1, X^+_1)  = H(z_1) - H(Z_1|f(Z, X^-))        
%     \end{split}
% \end{align}


% Currently, our agent predicts $X^+ \sim P(X^+|X^-, Y^-; Z)$ and the opponent predicts $Y^+ \sim P(Y^+|X^-, Y^-, X^+; W) = \frac{P(Y^+, X^+|X^-, Y^-; W)}{P(X^+|X^-, Y^-)} $


% Multi agent dynamics:
% $x_{t+1},y_{t+1} = f(x_t, y_t, u_t, v_t, w_t)$, where $w_t$ is noise. 
% This is equivalent to writing $P(x_{t+1},y_{t+1}|x_t, y_t, u_t, v_t)$. If $v_t \sim \pi_y$, then
% $P(x_{t+1},y_{t+1}|x_t, y_t, u_t) = \sum_{v_t}P(x_{t+1},y_{t+1}|x_t, y_t, u_t, v_t)\pi_y(v_t)$. 

% And $P(x_{t+1},y_{t+1}|x_t, y_t, u_t) = P(y_{t+1}|x_{t+1},x_t, y_t, u_t)P(x_{t+1}|x_t, y_t, u_t)$.

% Assuming that actions only control single agents, $P(y_{t+1}|x_{t+1},x_t, y_t, u_t) = P(y_{t+1}|x_{t+1},x_t, y_t)$, so 

% $$P(x_{t+1},y_{t+1}|x_t, y_t, u_t) = P(y_{t+1}|x_{t+1},x_t, y_t)P(x_{t+1}|x_t, y_t, u_t)$$
%%%%%%%%%%%%%%%%%

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.235\textwidth}
        \includegraphics[width=\textwidth]{cond_bumper.png}
        \caption{Conditional model}
        \label{fig:conditional}
    \end{subfigure} %\hspace{0.05\textwidth}
    \begin{subfigure}[b]{0.235\textwidth}
        \includegraphics[width=\textwidth]{dis_bumper.png}
        \caption{Disentangled model}
        \label{fig:disentangled}
    \end{subfigure}
    \caption{Comparison between disentangled and conditional models on box bumper domain. Blue agent ($x$) attempts to reach the target location below the horizontal obstacle (green circle), 
    % while receiving negative reward for leaving the play area, and 
    possibly being blocked by the red agent ($y$) in the narrow passage. Numbers indicate the segment order in time. Fig.~\ref{fig:conditional} shows a trajectory predicted by the conditional model. Since $x$ is independent of $y$, which only `responds' to its actions, the optimization cannot imagine a trajectory for which $x$ is blocked by $y$ en route to the goal, even in the worst case (risk-averse optimization). In fig.~\ref{fig:disentangled}, a sample is shown from the predictions of the disentangled model, where $x$ chooses to go left, since it assumes $y$ will block it in the right passage.}
    % $x$'s path and prevent it from receiving its reward.  } 
    \label{fig:bumpers}
    \vspace{-1em}
\end{figure}

\section{Model Architecture}

We now discuss the implementation details of our approach for solving the multi-agent problem defined above. In this section, we describe the data collection process, model architecture and training, and how we use the learned models for optimization in the latent space.

\subsection{Data Collection}
In this work, we follow the approach of \citet{mishra2017prediction}, and assume that data for training the dynamics model is generated from a predefined exploration policy. This policy should be diverse enough to `cover' the interesting strategies that the model can learn. For the multi-agent case, we assume that we have an exploration policy both for the agent $x$ and for the adversary $y$. 
% In many model-based RL studies, the policy that was learned by the model was used to generate additional data in an iterative optimization formulation~\citep{kurutach2018model}. We leave this study to future work, and 
We note that in our experiments, designing a suitable exploration policy was relatively straightforward, by stochastic action selection with some heuristic direction.

\subsection{Models and Training}
Following the two approaches described in Sec.~\ref{sec:matsm}, we train a separate TSM for each agent in the conditional model, and a shared TSM with a disentangled latent space for the disentangled model. All models are based on the architecture described by \citet{mishra2017prediction}, using CVAEs with dilated causal convolutions in both encoder and decoder. Full implementation details are in the supplementary material. 

% Recall that in our setting we have a controlled agent $x$ and a non-controlled agent $y$, which can act as an adversary to $x$. To capture this relationship between the agents, we allow the model for $y$ to observe the actions of the controlled agent $x$ in a non-causal manner (i.e. they 'respond' to the actions of other agents). This allows us to predict the possible reaction of $y$ to the strategy of $x$. Concretely, assume the segments of observations for the controllable agent are given by $X^-, X^+$ for past and future observations respectively, and the segments for the other agent are given by $Y^-, Y^+$. The decoder of the controllable agent predicts $\hat X^+ \sim \mathcal{P}(X^+|X^-, Y^-; Z)$ while the responsive model for the second agent predicts $\hat Y^+ \sim \mathcal{P}(Y^+|Y^-, X^-, X^+; W)$, where $Z$ and $W$ are the latent variables controlling both models, respectively. A more detailed comparison of the architectures can be found in the supplementary material. 
% To train our TSMs, we organize our data into consecutive past and future segments of both agents $(X^-, Y^-), (X^+, Y^+)$, and optimize the variational lower bound \eqref{eq:elbo} using the Adam optimizer. Full implementation details can be found in the supplementary material.  

\subsection{Multi-Agent Trajectory Optimization}

% As noted above, the motivation for learning a dynamics model is to later use this model to find an optimal solution for a task in the environment. 
% In addition, trajectory optimization is a useful tool for measuring the performance of our model. Poorly trained or insufficient models tend to produce predictions which are unrealistic in the real environment -- which leads to sub-optimal solutions of the optimization problem.

% Assume that the total horizon of interest $T$ can be segmented into $k$ segments of length $H$. Then, the learned models for future segment distributions $\mathcal{P}(X^+|X^-, Y^-; Z)$ and $\mathcal{P}(Y^+|Y^-, X^-, X^+; W)$ can be rolled-out $k$ times to produce a distribution for a $T$-length trajectory for both agents $x_0,y_0,\dots,x_{T},y_{T}$.
% For each $i \in 1,\dots, k$, we denote by $x^{+,i} = x_{i H : (i + 1) H - 1}$ and $x^{-,i} = x_{(i - 1)H:iH - 1}$ the $i^{\text{th}}$ future and past segments for agent $X$ in this rolled-out trajectory. Similarly, for the non-controlled agent $y$, we denote $y^{+,i} = y_{i H : (i + 1) H - 1}$ and $y^{-,i} = y_{(i - 1)H:iH - 1}$. We also denote by $z^{i}$ and $w^{i}$ the $i^{\text{th}}$ samples of the latent variables $Z$ and $W$ used to roll out each segment in the trajectory.

Recall that in our problem formulation, we seek to find a risk-sensitive policy against the probabilistic behavior of the opponent $y$ (see Sec.~\ref{sec:risk}). 
% Our idea is that the learned model for the non-controlled agent $\mathcal{P}(Y^+|Y^-, X^-, X^+)$ can be used to model the possible behaviors of $y$. 
Therefore, we propose the following trajectory optimization problem:
\begin{align} 
    \begin{split}
    \min_{z^{1},...,z^{k}} &\mathbb{E} \left[\left. \sum_{t=0}^{T} r_x(x_{t}, y_t) \right| \sum_{t=0}^{T} r_x(x_{t}, y_t) \leq Q_\alpha \right] \\
    \textrm{s.t. } &x^{+,i},y^{+,i} = f^{(x,y)}(x^{-,i}, y^{-,i}, z^{i}, w^{i}), \forall i\in 1,\dots,k\\
    % &y^{+,i} = f^{(y)} (y^{-,i}, x^{-,i}, x^{+,i}, w^{i}),\quad \forall i\in 1,\dots,k\\
    & w^{i} \sim \mathcal{P}_{prior}(W),\quad \forall i\in 1,\dots,k ,
    \end{split}
    \label{eq:opt_expected_adv}
    \raisetag{50pt}
\end{align}
The function $f^{(x,y)}$ denotes the CVAE decoder, and depends on the type of model used. 
For the disentangled model, it is the decoder for both $x$ and $y$, while for the conditional model, each agent has its own decoder (cf. Section \ref{sec:cond_msgm}).
Note that this is a formulation of problem~\eqref{eq:traj_opt_multi} for our case, with notation following the setting described in Sec.~\ref{sec:risk}. 
% This formulation works for both settings proposed in Sec.~\ref{sec:matsm}: when using conditional multi-step generative models, $f^{(x)}$ and $f^{(y)}$ are the decoders of two separate models, where the model for $y$ depends on future observations of $x$; while in the disentangled setting, $f^{(x)}$ and $f^{(y)}$ are both implemented by the same model, with $z$ and $w$ the disentangled parts of the same latent space.
% where $Q_\alpha$ denotes the $\alpha$-quantile of $\sum_{t=0}^{T} r_x(x_{t}, y_t)$.
% Note that here, compared to the original TSMs, we are optimizing over the the latent space of the controlled agent $x$, but \emph{marginalizing} over the latent space of the non-controlled agent $y$. By controlling the risk sensitivity, we can tune our belief towards $y$ -- a risk-averse attitude (i.e., a small $\alpha$) will assume that $y$ will act against us, while a risk seeking behaviour (which can be achieved by replacing $\leq$ with $\geq$ in the objective) assumes that $y$ will act in our favor. Setting $\alpha=1$ will result in an agent that optimizes against the expected behavior of $y$, as displayed in the collected data.

% Note also that this setup can be extended to any number of agents, with one agent responding with its 'best option' for the average trajectories of other agents. See the next section for examples of optimization using this paradigm. 

To practically solve problem \eqref{eq:opt_expected_adv}, we use a combination of sampling and gradient descent. It is well known that the CVaR (or the CVaR gradient) at level $\alpha$\% of a random variable $\Xi$ can be estimated by taking $m$ samples of $\Xi$, and averaging the smallest $\alpha$\% of the samples (or their gradient)~\citep{hong2009simulating}. Thus, we can replace the expectation in \eqref{eq:traj_opt_clean} with an average of the $\alpha$\% smallest values of $\sum_{t=0}^{T} r_x(x_{t}, y_t)$, where the sample comes from sampling the $w^{i}$ values from $\mathcal{P}_{prior}(W)$. This results in a deterministic optimization problem, which we can solve using gradient descent. In our implementation, we used Adam~\citep{kingma2014adam}, with multiple restarts from random initial values of $z^{1},...,z^{k}$, sampled from $\mathcal{P}_{prior}(Z)$. Detailed pseudocode is given in the supplementary material (see Alg.~\ref{alg2}).

\subsection{Trajectory Execution}\label{sec:traj_execution}

The trajectory optimization described above can only solve for a \emph{desired} trajectory in state space for our agent $x$. However, to execute the trajectory in the system, we need to select actions that `carry out' the imagined future steps. Here, we exploit the fact that in many systems, designing a tracking controller can be much simpler than designing a full policy~\citep{schaal2006dynamic}.

We propose to use the training data to also learn, in addition to the TSM models, an inverse dynamics model $P(u_t|x_t,x_{t+1})$. Using such a model, and the predicted state sequence for the agent $x_0,\dots,x_T$ (the result of trajectory optimization), we can compute actions that execute the desired trajectory.
Training an inverse dynamics model is a standard supervised learning problem, and in our experiments we found that standard multi-layered perceptrons (MLPs) work well.
To execute a full trajectory in the system, we adopt a model predictive control approach (MPC,~\citealt{nagabandi2017neural}): at the beginning of each segment $i$, we solve the trajectory optimization problem for the remaining segments $i,i+1,\dots,k$, starting from the current state of the agents, to obtain the desired trajectory for the agent at the current segment $x^{+,i}$. We then use the inverse model to track this trajectory segment. Then, at segment $i+1$, we observe the current position of the agents, solve the trajectory optimization again for the remaining $i+1,\dots,k$ segments, and repeat. This approach reduces the effect of drift from the imperfect inverse model, and also updates the controllable agent $x$'s policy against the real observations of the non-controlled agent $y$.

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.235\textwidth}
        \includegraphics[width=\textwidth]{temp_seg_7771.png}
        \caption{TSM trajectory (risk neutral)}
        \label{fig:tsm_traj}
    \end{subfigure} %\hspace{0.05\textwidth}
    \begin{subfigure}[b]{0.235\textwidth}
        \includegraphics[width=0.975\textwidth]{single_step_7771.png}
        \caption{Single step baseline}
        \label{fig:ssb_traj}
    \end{subfigure}
    \caption{Predator-Prey domain. The predator (blue) attempts to reach the escaping target (red) around the obstacle in the middle of the field.
    (a) Trajectory optimization for TSM using the risk-neutral setting ($\alpha=1$). (b) Trajectory optimization for the single step baseline. In both cases, the chasing agent (blue) starts to the left of the wall, while the target (red) starts to the right across from it. The trajectories are marked at every tenth step to enable temporal comparison, which coincides with the segment lengths for the TSM case. Both models imagine a successful chase of the prey. However, the TSM trajectory successfully circumvents the obstacle to reach the expected average location of the prey, while the baseline exploits an error in the the single step model and completely ignores the wall, which would fail at execution.} \label{fig:fc_traj_opt}
    \vspace{-1em}
\end{figure}

\section{Experiments}
To test our models, we use simulators and data collected from two domains:
% four multi-agent games. The first is a box environment, with one agent attempting to reach a goal location, while the other tries to block its path. The second and third tasks are set in a simple predator-prey scenario designed using
Multi-Agent Particle Environments -- a standard benchmark for multi-agent RL~\citep{lowe2017multi}, 
% A single agent tries to reach a target around an obstacle, while the target escapes in an adversarial manner. The fourth, more complex domain is
and 2D RoboCup Soccer Simulation \citep{kitano1997robocup,kalyanakrishnan2006half}.
% with two offensive players attempting to score against a defender and a goalkeeper.
% details for both of which are described below.

\subsection{Multi-Agent Particle Environments}\label{sec:particle}
Multi-Agent Particle Environments are a highly versatile RL playground, proposed by \citet{mordatch2017emergence} and used extensively in other work (e.g., \citealt{lowe2017multi}). The Particle Environment world allows for an arbitrary number of interacting agents, with user defined state and action spaces, and a highly configurable set of landmarks. For our experiments, we designed three simple environments: 

\textbf{(1)~Box-bumper:} a small, closed world where one agent attempts to reach a specified location behind an obstacle, while the other agent attempts to block it (see fig.~\ref{fig:bumpers}). 
\textbf{(2)~Predator-prey:} similarly to the scenario created by \citet{lowe2017multi}, a single agent chases an escaping target around an obstacle (see fig.~\ref{fig:fc_traj_opt}). Predator reward is negative distance to the prey.
% , while the prey attempts to maximize the same distance.
\textbf{(3)~Safe zone predator-prey:} modification of the previous environment, where prey has a `safe zone' at the bottom right corner of the game (see fig.~\ref{fig:fc_cvar})

The data we collected to train the world model for all multi-agent particle environment domains consists of 30k trajectories of 50 steps each, where the agent applies 5 steps in a random direction, then continues to move with inertia, selects a new direction and repeats. This type of exploration provides trajectories which are relatively evenly distributed around the playing field, along with a sizable percentage of collisions with the obstacles, which are important for learning an accurate world model.

\begin{table}
    \caption{Results (average distance to prey, lower is better) for predator-prey domain using a trajectory optimization policy. Each row represents a different initial setup of predator and prey relative to the wall obstacle. The results were obtained by averaging over 20 trajectories starting on the same side, and 60 from different locations on different sides. Our model outperforms the single-step baseline and the original exploration policy from both locations, with a larger advantage when the agents start on different sides of the wall (harder scenario). \\ }
    % \begin{tabular}{c|c||c|c|c}
    %  \textbf{Agent} & \textbf{Target} & \textbf{TSM} & \textbf{Single} & \textbf{Random} \\
    %  \textbf{Location} & \textbf{Location} &  & \textbf{Step} & \\
    %  \hline
    %  $[0.4, 0.3]$ & $[0.4, -0.3]$ & \textbf{0.7204} & 0.9223 & 1.5512 \\
    %  \hline
    %  $[-0.4, 0.0]$ & $[0.3, -0.1]$ & \textbf{0.8647} & 1.3451 & 1.8296 \\
    %  \hline
    %  $[0.2, 0.0]$ & $[-0.3, 0.3]$ & \textbf{0.9294} & 1.1825 & 1.6525 \\
    %  \hline
    %  $[0.2, 0.0]$ & $[-0.2, 0.0]$ & \textbf{1.0173} & 1.1551 & 1.6395 \\
    %  \hline
    %  $[0.4, 0.3]$ & $[-0.3, 0.2]$ & \textbf{0.9832} & 1.3319 & 1.7636
    %  \end{tabular}
    %  \label{tab:fc_opt_res}
    \begin{tabular}{c||c|c|c}
     \textbf{Locations} & \textbf{TSM (Ours,} & \textbf{Single} & \textbf{Random} \\
     \textbf{(Relative to wall)} & \textbf{risk neutral)} & \textbf{Step} & \\
     \hline
     Same side & \textbf{0.7204} & 0.9223 & 1.5512 \\
     \hline
     Different sides & \textbf{0.9486} & 1.2537 & 1.7213
     \end{tabular}
     \label{tab:fc_opt_res}
     \vspace{-2em}
\end{table}

\subsubsection{Box Bumper Domain}
The box bumper domain consists of a square playing area, with a horizontal wall set in the bottom half of the field. Two agents, which are relatively large compared to the area of interest, move around the field by applying forces in one of the four cardinal directions. Due to the limited size of this domain, the agents tend to collide often and block each other's way. 
%% OK: we can move this to the supplementary
% In this domain, we used the data collection policy described above, modified such that the random direction selection is weighted towards the location of the other agent to promote collisions between the agents, which are an area of interest in the state space.
The task of one agent in this environment is to reach the goal location, which is located below the middle of the wall. The other agent may attempt to block its path. 

The experiments in this domain are qualitative in nature, and serve as an example to the case where the conditional multi-step generative model (see Sec.~\ref{sec:cond_msgm}) may not be suitable, and the disentangled models (see Sec.~\ref{sec:disentangled}) may be necessary for a correct solution. We trained two multi-agent TSMs on this domain: the first was trained in the conditional form, where one controlled agent attempts to reach the goal, and the second agent plans trajectories conditioned on the path of the first; a second, disentangled model was trained using the mutual information maximization technique. 
%% OK: supplementary
% The observation space included the locations and velocities of both agents.
Fig.~\ref{fig:bumpers} presents the results of trajectory prediction using both models.

\begin{figure}
    \centering
    % \begin{subfigure}[b]{0.23\textwidth}
    %     \includegraphics[width=\textwidth]{pess773p.png}
    %     \caption{TSM trajectory (risk averse)}
    %     \label{fig:pessTSM}
    % \end{subfigure}
    % \begin{subfigure}[b]{0.23\textwidth}
    %     \includegraphics[width=\textwidth]{opt776p.png}
    %     \caption{TSM trajectory (risk seeking}
    %     \label{fig:optTSM}
    % \end{subfigure}
    \includegraphics[width=0.48\textwidth]{opt-pess_same_scale.png}
    \caption{Predator-Prey domain, with a safe zone for prey. The predator agent (blue, starts to the left of the obstacle) attempts to reach the prey (red, starts to the right), while the prey has a `safe zone' (marked by the green box) where the predator gets no reward for capturing it (and consequentially, the prey's reward grows). 
    Left: A risk-averse optimization, selecting the worst-case target trajectories and therefore anticipating that the prey goes towards the safe zone. Right: An optimistic optimization, where the best case prey trajectory moves away from the safe zone. } \label{fig:fc_cvar}
    % \vspace{-3em}
\end{figure}

\subsubsection{Predator-Prey}\label{sec:pred_prey}
The predator-prey domain simulates a chase scenario, with one agent chasing the other around a vertical wall obstacle. The cost incurred by the agent is the sum of distances between the agent and target along a complete trajectory.
%% OK: supplementary
% The observation space for each agent consists of the agent location, its velocity and the vector from the agent to the center of the wall. 
% We used the same learned model for both agents $x$ and $y$ when conducting trajectory optimization.

Data was collected with the exploration policy described above. Using the collected data, we trained two world models: a TSM and a single-step MLP dynamics model to serve as a baseline for comparison. We used both learned models to optimize over trajectories as described above (see Alg.~\ref{alg2} in the supplementary material). Despite exploring multiple network architectures and conducting a hyper-parameter search, none of the single step baselines we trained were able to correctly predict collisions with the wall. This enabled the baseline agent to exploit the failures of the model when optimizing for the best trajectories, as can be seen in fig.~\ref{fig:fc_traj_opt}. The same figure shows the success of our model in the same case. We compared the models quantitatively by executing their optimized trajectories in the simulator using MPC, playing against a target which used the aforementioned exploration policy. A comparison of the performance of the different models can be seen in Table~\ref{tab:fc_opt_res}.

\begin{table}
    \centering
    \caption{Results (average distance considering safe zone, lower is better) for the safe-zone predator-prey domain. The comparison was made by playing 100 scenarios starting from random starting locations, and averaged over 3 random seeds. \\}
    \begin{tabular}{c||c}
     \textbf{Optimization Method} & \textbf{Cost} \\
     \hline
     Risk averse (Worst case) & \textbf{0.9647} \\ %0.9682, 0.9358, 0.9894 
     \hline
     Risk neutral (average) & 1.0574 % 1.0508, 1.0689, 1.0452
     \end{tabular}
     \label{tab:fc_cvar}
\end{table}
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.22\textwidth}
        \includegraphics[width=0.85\textwidth]{real3.png}
        \caption{Baseline: captured ball}
        \label{fig:real3}
    \end{subfigure} %\hspace{0.05\textwidth}
    \begin{subfigure}[b]{0.22\textwidth}
        \includegraphics[width=0.85\textwidth]{imagined3.png}
        \caption{Predicted: goal}
        \label{fig:im3}
    \end{subfigure}
    \begin{subfigure}[b]{0.22\textwidth}
        \includegraphics[width=0.85\textwidth]{real15.png}
        \caption{Baseline: out of time}
        \label{fig:real15}
    \end{subfigure} %\hspace{0.05\textwidth}
    \begin{subfigure}[b]{0.22\textwidth}
        \includegraphics[width=0.85\textwidth]{imagined15.png}
        \caption{Predicted: goal}
        \label{fig:im15}
    \end{subfigure}
    \caption{Trajectory optimization in the HFO domain. Trajectories (a) and (c) are real trajectories of the hand coded Agent2D, while (b) and (d) are the respective optimized trajectories predicted by our model. Blue and Cyan denote the (controlled) offense players, Red denotes the (uncontrolled) defense player and goal keeper, and Purple denotes the ball. In both cases, our model improves the result -- in (a), while Agent2D kicks the ball towards the goalkeeper, our model aims toward the free side of the goal (b). In (c), Agent2D runs out of time to score, while our model predicts a more efficient trajectory (d). 
    % Note that even though our predictions for the ball are somewhat jagged, it still remains close to the distribution of the data and does not diverge too far from its realistic path. 
    }
    \label{fig:hfo_traj_opt}
    \vspace{-1em}
\end{figure}

\subsubsection{Safe Zone Predator-Prey}
% Using the same trained model\footnote{This also shows the power of model-based RL: without re-training the model, the agent optimizes for a new task successfully having never seen it before.}, we modified the task of the predator-prey environment by changing the cost function. 
In this scenario, there exists an area where the predator incurs no reward for being near the prey, and the prey is not penalized for the predator being close to it. This scenario is ideal for conducting CVaR optimization, the results of which we show in fig.~\ref{fig:fc_cvar}. Comparing the various cases, it is clear that risk-averse or risk-seeking optimization leads to either competitive or cooperative behavior, respectively. 

% OK: Consider removing both this and the table it refers to. Results are not as "impressive" as the other table, and are clearer in the visual figure. Might be a good space saver...
In addition to the visual results in fig.~\ref{fig:fc_cvar}, we tested the model over 100 episodes with random starting locations for predator and prey, with the predator using the learned TSM, and the prey escaping using a worst-case selection from the exploration policy. Table~\ref{tab:fc_cvar} compares the results of trajectory optimization when optimizing for the risk-averse (worst case) and the neutral (average) behavior of the prey. The results show clearly that using a risk-averse optimization scheme fares better against an adversarial opponent.



\subsection{RoboCup 2D Simulation}\label{sec:hfo}

RoboCup \citep{kitano1997robocup} is a well-known and diverse robotic soccer domain, which poses a challenge for many fields of research, from robotics to RL. The RoboCup 2D Soccer Simulation is a subdomain of RoboCup which focuses on agent strategy and cooperation. We use the Half Field Offense (HFO) environment \citep{kalyanakrishnan2006half,barrett2017making}, which is based on RoboCup 2D Simulation, to test our method in a challenging multi-agent environment. The scenario we play is a 2 vs. 2 game, where two offensive agents holding the ball attempt to score against a defender and a goalkeeper. The game ends when either a goal is scored, the defense touches the ball, the ball goes out of bounds or a certain time limit is reached. 

The exploration policy we use to collect data for the HFO domain is a hand coded one, native to the RoboCup simulator, named Agent2D. 
% Agent2D uses heuristics of distances between agents and open angles towards the goal to decide when to dribble the ball, pass it to other players or shoot it. 
We collected 17k trajectories of Agent2D agents playing against each other, where the observation space includes the locations and velocities of all agents and the ball, as well as player distance from the ball. 

Using this data, we trained TSMs for the various agents (see implementation details in the supplemental material). Rather than creating a model for each player separately, we consider the offense agents as one player ($x$) and the defense players as the adversary ($y$). Looking at both offensive players as a single agent allows us to plan a strategy for the entire offense, and does not limit us to the local actions of each player. The model for the offensive agent predicts the dynamics of the whole game, while the adversarial model is conditioned on the offense segment, following the conditional setting described in Sec.~\ref{sec:cond_msgm}. 
% An additional feature of the HFO domain is the ball, which does not select its own actions but responds to the actions of both offense and defense players. To model its behavior, we use a deterministic architecture based on the TSM decoder. 

Using the models learned from this dataset, we perform trajectory optimization for the task of scoring a goal. We incur a cost of 0 when a goal is scored and 1 for each time step without a goal. 
% This formulation not only promotes goal scoring, but also pushes the agent to score sooner in the game.
Using trajectories optimized for this task, our models predict scoring in scenarios where the Agent2D policy fails to do so (starting from the same initial positions). Due to technical difficulties with the HFO domain (such as inaccurate state information) we were not able to execute predicted trajectories in the simulator. Therefore, our results are qualitative examples (in fig.~\ref{fig:hfo_traj_opt} and the supplementary material) demonstrating multi-agent optimization. 

An additional observation arising from the HFO experiments is that the resulting latent space does indeed encode a strategy space, as different areas in the latent space correspond to different offensive strategies -- see fig.~\ref{fig:hfo_strategies} and the supplementary material for examples. 
% We leave further exploration of the structure of the latent space for future work. 

\section{Conclusion}
% TODO: the conclusion is going to be different from the one in the AAAI submission; needs rewriting

% TSMs are a promising approach to model based RL, which circumvent challenges like the accumulation of error when rolling out model predictions, and the tendency of the optimization to exploit errors in the model. 
In this work, we extended the idea of multi-step generative models to handle multi-agent problems, building on risk-sensitive optimization and sampling. We have applied our two suggested methods, of disentangled mutual information models and conditional models, to two domains, a predator-prey game (with several sub-tasks) and a simulated RoboCup environment. Our results show that the multi-agent TSM models effectively capture a reasonable `strategy space' of the agents, and that optimization in this space leads to realistic plans for execution. This results in an effective and interpretable decision making algorithm.

% In future work, we will explore how to apply these ideas to domains with a large number of agents, and domains with more complex observation structure such as images.


\bibliography{references.bib}
\bibliographystyle{plainnat}

%% Comment out when generating PDF for submission
\clearpage

\appendix
\section{Training Algorithm}
The following algorithm is the training flow for our models. $\texttt{Enc}$ and $\texttt{Dec}$ are the encoder and decoder of the Conditional Variational Autoencoder, and their architecture depends on the specific model (see below). When training the conditioned model (see Sec.~\ref{sec:cond_msgm}, the decoder is also conditioned on $y^+$ and $y^-$.
$\texttt{InfoEnc}$ are additional encoders arising from the mutual information lower bound described by \citet{chen2016infogan}: 
\begin{align*}
    \begin{split}
        L_I&(f, Q) = \\
        &\mathbb{E}_{Z_1\sim P(Z_1),X^+_1\sim f(Z, X^-)}[\log Q(Z_1|X_1^+)] + H(Z_1) \leq \\ 
        & I(Z_1, f(Z, X^-)) = I(Z_1, X^+_1)
    \end{split}
\end{align*}
We model $Q(Z_1|X^+_1)$ as an additional encoder, which attempts to reconstruct $Z_1$ from $\hat X^+_1$ mentioned above. Since the prior for $Z$ (and consequently, $Z_1$ and $Z_2$) is fixed, we can ignore it and only optimize for the expectation term, which can be interpreted as the negative MSE between $Z_1$ and $Q(Z_1|\hat X^+)$.
We used three weighting factors ($\gamma, \lambda_1, \lambda_2$) to weight the different parts of the loss function. We find that some hyper-parameter tuning on those coefficients is needed to receive working models. 
\begin{algorithm}
    \caption{Multi-Agent Multi-Step Generative Model Training}
    \label{alg1}
    \begin{algorithmic}[1]
        \STATE $\mathcal{D}\leftarrow \{(x^-,x^+)\}_{i=1}^N$ Initialize dataset with pairs of matching past and future segments
        \STATE $B, \texttt{Enc}, \texttt{Dec}, opt\leftarrow$ Initialize batch size, model (encoder and decoder) and optimizer
        \STATE $\gamma, \lambda_1, \lambda_2 \leftarrow $ Initialize loss weighting parameters
        \IF {Disentangled model}
            \STATE $\texttt{InfoEnc}_{1,2} \leftarrow $ Initialize encoders for mutual information maximization
        \ENDIF
        \FORALL{epochs}
            \FORALL{samples of $B$ pairs in  $\mathcal{D}$}
                \STATE $\mu_z, \sigma_z = \texttt{Enc}(x^+)$
                \STATE Sample $\{z\}_1^B \sim N(0, I)$
                \STATE $\hat x^+ = \texttt{Dec}(x^-, z \cdot \sigma_z + \mu_z)$
                \STATE $\ell = \text{MSE}(\hat x^+, x^+) - \gamma \mathcal{D}_{KL}[\mathcal{N}(\mu_z, \sigma_z)||\mathcal{N}(0,I)]$ 
                \IF {Disentangled model}
                    \STATE $\ell \leftarrow \ell - \lambda_1 \text{MSE}(\texttt{InfoEnc}_1(x^+_{(1)}, z_{(1)}) - \lambda_2 \text{MSE}(\texttt{InfoEnc}_2(x^+_{(2)}, z_{(2)})$
                \ENDIF
                \STATE Backprop$(\ell)$
                \STATE opt.step()
            \ENDFOR
        \ENDFOR
        \STATE Return trained model
    \end{algorithmic}
\end{algorithm}

\section{Trajectory Optimization Algorithm}
We provide pseudo-code for our method. This version shows the optimization when using the conditional model (Sec.~\ref{sec:cond_msgm}), however, it can be easily modified for the disentangled model version (Sec.~\ref{sec:disentangled}) by replacing lines 11-12 with a draw from a single shared model.

\begin{algorithm}
    \caption{Multi-Agent Trajectory Optimization}
    \label{alg2}
    \begin{algorithmic}[1]
        \STATE $x_0, y_0\leftarrow $ Initialize agents' states
        \STATE $N, m, l, k \leftarrow$ initialize batch size (number of optimization restarts), non-controllable agent trajectory samples, latent dimension of $Z$, segments per game
        \STATE $a = \alpha m$ risk sensitivity
        % \FORALL{$i$ in game segments (MPC loop)} 
          \STATE $z \leftarrow$ initialize latent variable $(n \times k \times l )$ by sampling from $\mathcal{P}_{prior}(Z)$
          \STATE $w \leftarrow$ sample latent variable $(m \times k \times l )$ from $\mathcal{P}_{prior}(W)$
          \STATE opt $\leftarrow$ initialize  optimizer (Adam)
          \FORALL{restarts $i$ in $n$}
            \FORALL{epochs}
                \FORALL{samples $j$ in $m$}
                    \FORALL{game segments}
                        \STATE $x^+_{i,j} = f^x(x^-_{i,j}, y^-_{i,j}, z_i)$
                        \STATE $y^+_{i,j} = f^y(x^-_{i,j}, y^-_{i,j}, x^+_{i,j}; w_j)$
                    \ENDFOR
                    \STATE loss$_{i,j} = -r_x(x_{i,j}$, $y_{i,j})$ summed over all segments
                \ENDFOR
                \STATE Sort loss$_{i,j}$ in increasing order along $j$
                \STATE loss$_{i} = \frac{1}{a}\sum_{j=1}^{a} \text{loss}_{i,j}$
            \ENDFOR
            \STATE Backprop loss
            \STATE opt.step()
        % \ENDFOR
        \ENDFOR
        \STATE Return trajectory $x_{i,j}$ that corresponds to the lowest $i$ in loss$_{i}$ and the highest $j$ in loss$_{i,j}$
    \end{algorithmic}
\end{algorithm}

\section{Predictions from the Disentangled Model}
To ensure that our disentangled setting of the model learns representations where different parts of the latent space control different parts of the output (i.e. different players), we run a simple experiment: we set one part of the latent space ($z_1$) to a constant value, and sample from the prior distribution to obtain values for the other part ($z_2$). We then use this latent variable construct, along with past segments, to predict future segments using our decoder. We expect to produce trajectories where one agent acts in a deterministic manner (as given $Z$, $D(X^-, Z)$ is a deterministic function) and the other agent producing a distribution over possible trajectories. Fig.~\ref{fig:freeze} shows example results of this experiment. 

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{info_sep1.png}
        \label{fig:freeze1}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{info_sep2.png}
        \label{fig:freeze2}
    \end{subfigure}
    \caption{Two examples of the bumper box domain, sampled from the disentangled model with one part of the latent space 'frozen' (set to a constant value), and the other part sampled from the prior. As expected, the behavior displayed is deterministic for one player, and distributed for the other. Red marks the distributed predictions for one agent, caused by sampling its latent variable from the prior. Blue trajectories are the ones predicted when the latent variable is 'frozen', thus causing deterministic behavior. Magenta and cyan lines denote the original trajectories collected from data, for reference. } \label{fig:freeze}
    % \vspace{-3em}
\end{figure}

\section{Detailed Implementation Parameters for Bumper Box}
Data for the bumepr domain was collected using the exploration policy described in \ref{sec:particle}, modified such that the random direction selection is weighted towards the location of the other agent to promote collisions between the agents, which are an area of interest in the state space. The observation for each agent is the location and velocity of both itself and its counterpart.
Similarly to \citet{mishra2017prediction}, we used an encoder with two layers of dilated causal convolutions and Tanh activations, and a decoder with three dilated causal convolution layers and an additional 1-dimensional convolution at the output. The decoder activation functions are the same as suggested for this type of architecture \citep{van2016wavenet} and used by \citet{mishra2017prediction}:
\begin{align}
\tanh(W_{f,k} * s + V^T_{f,k}z) \odot \sigma(W_{g,k} * s + V^T_{g,k}z)
\end{align}
where $*$ denotes a convolution, $\odot$ is element-wise multiplication, $s$ is the output of the previous layer, $z$ is the latent variable and both $V$ and $W$ are learned weights. For the disentangled model (Sec.~\ref{sec:disentangled}), we added two additional encoder networks to enable mutual information maximization between parts of the latent space and corresponding parts of the output. 
We found that a segment length of 10 steps and latent spaces of dimension 8 or 12 were a good choice for accurately learning the environment dynamics. We trained our model with Adam for 2000 epochs, using the standard hyper-parameters.  

\section{Detailed Implementation Parameters for Predator Prey}
In this domain, we used a slightly different observation space, reflecting the fact that agents rarely interact and are dependent only in their reward. Each agent's observation space included its location, its velocity and a vector pointing to the middle of the obstacle. During training, we offset the agent location (but not the obstacle vector) by the first location in the segment. In this manner, we trained the same models for both predator and prey agents. 
Similarly to the bumper box domain, we used an 8-dimensional latent space and 10-step segments. As this domain is somewhat less complicated, training tended to converge faster (even though we used somewhat smaller batch sizes). All other architecture parameters were the same as described in the previous section. 
As described in Sec.~\ref{sec:pred_prey}, we also trained a single-step baseline for this scenario. After conducting an architecture search, we concluded that a fully-connected, 3-layer MLP performed as well as any of the other architectures, and used it as a baseline for its simplicity of implementation. 

\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.22\textwidth}
        \includegraphics[width=\textwidth]{strat12.png}
        \caption{Single player, left}
        \label{fig:strat_alone_top}
    \end{subfigure} \hspace{0.02\textwidth}
    \begin{subfigure}[b]{0.22\textwidth}
        \includegraphics[width=\textwidth]{strat14.png}
        \caption{Single player, right}
        \label{fig:strat_alone_mid}
    \end{subfigure} \hspace{0.02\textwidth}
        \begin{subfigure}[b]{0.22\textwidth}
        \includegraphics[width=\textwidth]{strat15.png}
        \caption{One pass}
        \label{fig:strat_pass_once}
    \end{subfigure} \hspace{0.02\textwidth}
    \begin{subfigure}[b]{0.22\textwidth}
        \includegraphics[width=\textwidth]{strat11.png}
        \caption{Two passes}
        \label{fig:strat_pass_twice}
    \end{subfigure}
    % \framebox[\columnwidth]{\rule{0pt}{160pt}}
    \caption{Plots of the trajectories predicted for four random latent variable draws. Blue and cyan lines are the two offense players (controlled by the agent) and red lines denote the defense players. The purple line denotes the ball. Trajectories are divided into segments of 10 time steps, and circles indicate the segment index. In~\ref{fig:strat_alone_top} the agent plans a strategy where the blue player advances alone and shoots the ball from the left. In~\ref{fig:strat_alone_mid} a different strategy arises, with the blue player dribbling the ball towards the right of the field and kicking from there. In~\ref{fig:strat_pass_once} the strategy is yet again different, and incorporates blue catching the ball and passing it to cyan, who in turn shoots. \ref{fig:strat_pass_twice} shows an altogether different strategy, in which the cyan player catches the ball and passes it to blue. }
    \label{fig:more_strategies}
\end{figure*}

\section{Detailed Implementation Parameters for HFO 2 vs. 2}
 As in the Multi-Agent Particle Environment, we found an 8-dimensional latent space and a 10-step segment were suitable to capture the dynamics. We also used a similar architecture to the one described above. However, we found we needed our models to be somewhat more expressive, and added channels to each convolution. Moreover, instead of predicting the next agent location directly, the models we trained for this domain predict the change in location and velocity, and add it to the previous known location to create future states. 
 Finally, for ease of training, we equalized the length of all collected data trajectories to 100 time steps, truncating longer ones and repeating the final state of shorter ones. This enables us to train without some sort of 'end scenario' signal.
 
 \section{Additional examples for Strategy Space Planning in HFO}
 As described in Sec.~\ref{sec:hfo} and demonstrated in Fig.~\ref{fig:hfo_strategies}, drawing different samples from the latent space can provide completely different \emph{strategies} for the offensive agents, and does not just affect the trajectory details. This can be clearly seen in fig.~\ref{fig:more_strategies}, in which each trajectory is the (non-optimized) result of different samples of the latent space, all from the same starting location. 

\end{document}


==> old_stuff.tex <==
\section{Move elsewhere}
Let us first consider the single agent scenario.
Consider the following continuous control problem:
% \begin{equation*}
$
    % \begin{split}
        \max_{u_0,\dots,u_T} \sum_{t=0}^T r(x_t,u_t) 
        s.t. \quad x_{t+1} = f(x_t, u_t)
    % \end{split}
$
% \end{equation*}
where $r(x_t,u_t)$ is a known reward function, and $x_{t+1} = f(x_t,u_t)$ represents the (deterministic) dynamics of the environment. We denote $R(x_0,u_0,\dots,x_T,u_T) = \sum_{t=0}^T c(x_t,u_t)$.
Now, assume we have some model for the trajectory with a parameter $z$, that is, we can write
\begin{equation*}
    x_0,u_0,\dots,u_T = G(z),
\end{equation*}
for some $z$, for any $x_0,u_0,\dots,u_T$.
Then, an equivalent optimization problem is 
\begin{equation*}
    \max_z C(G(z)).
\end{equation*}
Note that there is no restriction on the model here, except that there is a one-to-one mapping between the trajectory and $z$. In particular, the single step model fits this derivation, where in that case $z$ would trivially correspond to the sequence of actions $u_0,\dots,u_T$. However, when we learn the model from data, it might be that we want different representations.

%===============================================================================

% \section{Multi-Agent Multi-Step Generative Models}
\AT{Put competitive and cooperative here}
% In this paper, we consider an extension to the MDP model for a multi-agent setting known as a Markov Game~\cite{littman2001value}. For simplicity, we present the case of two agents, but our results can easily be extended to more players (e.g. as described by \citealt{littman2001value}). 
% Consider two agents $x$ and $y$ acting in a dynamic environment. At time-step $t$, the states of the agents are denoted by $x_t$ and $y_t$, respectively. The agents each select an action $a_t \in \mathcal{A}$ and $b_t \in \mathcal{B}$, out of their respective action sets. The dynamics of the environment are then governed by the distribution (or function) $\mathcal{P}(x_{t+1}, y_{t+1} \vert x_t, y_t, a_t, b_t)$, and the agents obtain rewards $r_x(x_t,y_t)$ and $r_y(x_t,y_t)$, respectively. This formulation can be used to define adversarial scenarios (e.g. by selecting zero sum rewards), cooperative scenarios (e.g. by selecting the same reward function for both agents), or various combinations thereof. To simplify our presentation, in this work we focus on the case of deterministic dynamics, given by $x_{t+1}, y_{t+1} = f(x_t, y_t, a_t, b_t)$.\footnote{An extension to stochastic dynamics can be done by adding another uncontrolled agent with action $c$ that represents noise, and writing the transition as $x_{t+1}, y_{t+1} = f(x_t, y_t, a_t, b_t, c_t)$. We leave a full investigation of stochastic dynamics to future work.}

%In our setting, we consider a case where only agent $x$ is controlled, while the policy and reward driving agent $y$ are not known. In particular, we do not assume that $y$ has any fixed behavior. 
In the two-player game scenario, We consider two settings: adversarial and cooperative. In the adversarial setting, $x$ assumes that $y$ acts to hinder our agent, and optimize a zero-sum game:
% \begin{equation*}
$
    \max_{\pi_x} \min_{\pi_y} \mathbb{E} \left[ \sum_{t=1}^{T} r(x_{t}, y_{t}) \right],
$
% \end{equation*}
where $\pi_x$ and $\pi_y$ denote the policies of $x$ and $y$, respectively.
In contrast, in the cooperative setting $y$ is assumed to have the same objective as $x$:
% \begin{equation*}
$
    \max_{\pi_x, \pi_y} \mathbb{E} \left[ \sum_{t=1}^{T} r(x_{t}, y_{t}) \right].
$
One can also consider middle grounds between the adversarial and cooperative settings, such as assuming that $y$ acts according to a fixed distribution. 
% Our work can easily be extended to such cases.
% \end{equation*}

Now, let's consider the two-player game setting, where we are interested in a max-min game.
\begin{equation}\label{eq:prob_uw}
    \begin{split}
        \max_{u_0,\dots,u_T} \min_{w_0,\dots,w_T}& \sum c(x_t,y_t,u_t,w_t) \\
        s.t. & \quad x_{t+1}, y_{t+1} = f(x_t, y_t, u_t, w_t).
    \end{split}
\end{equation}
We denote $C(x_0,y_0,u_0,w_0,\dots,u_T,w_T) = \sum c(x_t,y_t,u_t,w_t)$. Again, assume we have some model for the trajectory with a parameters $z_x,z_y$, that is, we can write
\begin{equation*}
    x_0,y_0,u_0,w_0,\dots,u_T,w_T = G(z_x,z_y).
\end{equation*}
In addition, assume that $z_y$ is independent of $u_0,\dots,u_T$. That is, $\frac{\partial u_0,\dots,u_T}{\partial z_y} = 0$, and similarly $z_x$ is independent of $w_0,\dots,w_T$.
Then we can optimize
\begin{equation}\label{eq:prob_z}
    \max_{z_x} \min_{z_y} C(G(z_x, z_y)).
\end{equation}
This is justified as follows. A saddle point of \eqref{eq:prob_z} satisfies $\frac{\partial C}{\partial z_x} = 0$ and $\frac{\partial C}{\partial z_y} = 0$. We will show that it is also a saddle point of \eqref{eq:prob_uw}. We have that
\begin{equation*}
    \frac{\partial C}{\partial z_y} = \frac{\partial C}{\partial u_0,\dots,u_T} \frac{\partial u_0,\dots,u_T}{\partial z_y} + \frac{\partial C}{\partial w_0,\dots,w_T} \frac{\partial w_0,\dots,w_T}{\partial z_y},
\end{equation*}
and therefore 
\begin{equation*}
    \frac{\partial C}{\partial w_0,\dots,w_T} \frac{\partial w_0,\dots,w_T}{\partial z_y} = 0.
\end{equation*}
So long as $z_y$ is not redundant, i.e., $\frac{\partial w_0,\dots,w_T}{\partial z_y}\neq 0$, we have that $\frac{\partial C}{\partial w_0,\dots,w_T}=0$. Following the same derivation for $z_x$, we obtain a saddle point for \eqref{eq:prob_uw}.
% Our goal is to optimize the sum of rewards for agent $x$ in these cases. In the remainder of this section, we first describe our optimization criterion, and later discuss how to learn suitable generative multi-step models in order to optimize it.

% \subsection{Risk-Sensitive Optimization Formulation}\label{sec:risk}
% \AT{Remove this}
% To solve the multi-agent decision problem above, we propose to learn a probabilistic model for the \emph{possible} behaviors of $y$, 
% % $\mathcal{P}(b|x,y)$, 
% as seen in the data, and optimize a \emph{risk-sensitive} behavior policy for $x$, where the risk attitude would correspond to our belief about the nature of agent $y$'s policy. In particular, we consider the conditional value at risk measure (CVaR, a.k.a.~expected shortfall, \citealt{rockafellar2000optimization}). The CVaR at level $\alpha$\% of a random variable denotes the expectation of the variable on the worst (or best) $\alpha$\% of cases. Intuitively, as we optimize for the worst (best) cases, we take into consideration the adversarial (cooperative) nature of the other agents in the game. This statement has been made concrete by \citet{artzner1999coherent}. In this work, therefore, we opt to maximize the risk-averse CVaR of agent $x$'s sum of rewards:  $\mathbb{E}\left[\left.\sum_{t=0}^T r(x_t,y_t)\right|\sum_{t=0}^T r(x_t,y_t) \leq Q_\alpha\right]$, where $Q_\alpha$ denotes the $\alpha$-quantile of the sum of rewards, and the expectation is taken with respect to agent $y$'s behavior. 
% % $\mathcal{P}(b|x,y)$. 
% Note that when $\alpha=1$, we obtain the expected sum of rewards, while for $\alpha \to 0$ we optimize for the worst case. \footnote{To maximize a risk-seeking agent, we consider  $\mathbb{E}\left[\left.\sum_{t=0}^T r(x_t,y_t)\right|\sum_{t=0}^T r(x_t,y_t) \geq Q_\alpha\right]$. In this case, $\alpha=0$ corresponds to the expected sum of rewards, while for $\alpha \to 1$ we optimize for the best case.}

% Solving the risk-averse optimization problem would correspond to planning for an adversarial $y$, while computing a risk-seeking behavior would correspond to the assumption that $y$ is cooperative. Solving for the expectation, in this case, would be a 'middle ground' between assuming that $y$ is adversarial or cooperative. We next discuss how to learn suitable models for the behavior of $y$.


Latent spaces in multi-step generative models are generally unstructured \cite{mishra2017prediction,rhinehart2018deep}, and cannot be queried to control various aspects of the predicted segment. Here, we propose a representation where the elements of the latent space are \emph{disentangled} with respect to their effect on the two agents' strategies. That is, some elements in the latent space control the strategy of agent $x$, while other elements control the strategy of $y$.
% Such a "seperability" property would be extremely helpful when optimizing models for multiple agents, as each part of the latent space could be trained to control the future trajectories of different agents. 
% We borrow ideas from \citet{chen2016infogan} and \cite{klys2018learning}, where the latent spaces of generative models are partitioned to control various aspects of the generated output. 

To learn such a representation, we borrow ideas from \citet{chen2016infogan} and \citet{klys2018learning}, and propose to use the notion of mutual information to induce dependency between elements in the latent space and desired elements in the predicted trajectory. 

The mutual information between random variables $Q$ and $V$ is:
% \begin{equation*}
$
    I(Q;V) = H(Q) - H(Q|V) = H(V) - H(V|Q),
$
% \end{equation*}
where $H(Q)$ denotes the entropy of $Q$, and $H(Q|V)$ denotes the conditional entropy~\cite{cover2012elements}. Following the discussion above, to induce a disentangled latent representation for $X$ and $Y$ we would like to maximize the mutual information between $Z$ and $X$, and between $W$ and $Y$. We therefore propose the following loss function for training the generative model:
\begin{equation}\label{eq:loss_info}
    \min_\theta \mathcal{L} - \lambda_1 I(Z; X^+) - \lambda_2 I(W; Y^+)
\end{equation}
where $\mathcal{L} = \mathbb{E}_{Z,W\sim Q} \left[\log P(X^+,Y^+|X^-,Y^-,Z,W)\right] - \mathcal{D}_{KL}\left[Q(Z,W|X^+,Y^+)||P_{prior}(Z,W)\right]$ is the evidence lower bound~\cite{kingma2013auto}, and $\lambda_1>0$ and $\lambda_2>0$ are weights on the mutual information terms. To optimize \eqref{eq:loss_info} in practice, we use the lower bound proposed by \citet{chen2016infogan} We provide a full algorithm (Alg.~\ref{alg1}) in the supplementary material.
% and a part of the output future prediction, $X^+_1$ (completing the notation from the previous subsection). 
% Therefore, incorporating our variational lower bound from eq.~\eqref{eq:elbo}, the optimization objective of learning our model becomes: 
% \begin{align}
%     \min_\theta \mathcal{L} - \lambda I(Z_1, X^+_1) 
% \end{align}
% As noted by \citet{chen2016infogan}, in practice, maximizing the mutual information term directly is hard, since it requires access to the posterior $\mathcal{P}(Z|X^+)$. We can instead lower bound the information term using Variational Information Maximization \cite{agakov2004algorithm}. As shown by \citet{chen2016infogan}, the lower bound can be written as:
% \begin{align}
%     \begin{split}
%         L_I(f, Q) &= \mathbb{E}_{Z_1\sim P(Z_1),X^+_1\sim f(Z, X^-)}[\log Q(Z_1|X^+)] + H(Z_1) \leq \\ 
%         &\leq I(Z_1, f(Z, X^-)) = I(Z_1, X^+_1)  = H(z_1) - H(Z_1|f(Z, X^-))        
%     \end{split}
% \end{align}

\subsubsection{Conditional Multi-Step Generative Models} \label{sec:cond_msgm}
An alternative disentangled model representation can be obtained by conditioning. Since $P(X^+,Y^+|X^-,Y^-)=P(X^+|X^-,Y^-)P(Y^+|X^-,Y^-,X^+)$, we can learn two independent models: one for $P(X^+|X^-,Y^-)$ with a latent variable $Z$, and one for $P(Y^+|X^-,Y^-,X^+)$ with a latent variable $W$. Such will guarantee that the latent variables $Z$ and $W$ represent the strategies of $X$ and $Y$, respectively. However, such a formulation is not necessarily compatible with our CVaR optimization approach.

Since we are optimizing over $Z$, and $P(X^+|X^-,Y^-)$ does not depend on the value of $W$, we are effectively letting agent $x$ `play first', and choose its trajectory, while agent $y$ can only react to the trajectory of $x$ that has already been chosen.\footnote{Conversely, if we model the distribution as $P(Y^+|X^-,Y^-)P(X^+|X^-,Y^-,Y^+)$, we are giving an advantage to player $y$.} This advantage to player $x$ is demonstrated in simple blocking example in Figure \ref{fig:cond_illustration}, and also in our experiments (see fig.~\ref{fig:bumpers}). 

However, the conditional representation is still appropriate under some conditions. Consider a system where the dynamics of the agents are independent, i.e., can be written as $x_{t+1} = f_x(x_t, a_t)$ and $y_{t+1} = f_y(y_t, b_t)$, while the coupling between the agents is realized only through the reward function $r(x,y)$. In such cases, learning two independent models for the agents is compatible with the CVaR optimization. While this representation is limited in its applicability, its simplicity is an advantage in practice and, as we show in our experiments, it is suitable for several interesting domains such as the RoboCup simulation.

% The below is math we wrote a few months ago, which may describe the model a little better than the paragraph below it (of course we'll still need the CVaR parts)
% Is the conditional model always enough? Can we think of a scenario where we need a shared model for different agents? \\
% $P(x,y) = P(x|y)P(y)$ \\

% \subsection{Information Theoretic Generative Models}
% Latent spaces in multi-step generative models are generally unstructured \cite{mishra2017prediction,rhinehart2018deep}, and cannot be queried to control various aspects of the predicted segment. Such a "seperability" property would be extremely helpful when optimizing models for multiple agents, as each part of the latent space could be trained to control the future trajectories of different agents. We borrow ideas from \citet{chen2016infogan} and \cite{klys2018learning}, where the latent spaces of generative models are partitioned to control various aspects of the generated output. 

% We propose to use the notion of mutual information \eqref{eq:mut_inf} to enforce a relation between parts of the latent space and parts of the output variable. A general definition of mutual information is given by: 
% \begin{align}
%     I(X;Y) = H(x) - H(X|Y) = H(Y) - H(Y|X)
% \end{align}
% Where $H(X)$ denotes the entropy of a random variable $X$, and $H(X|Y)$ denotes the conditional information. In our case, we'd like to maximize mutual information between a part of the latent space, denoted by $Z_1$, and a part of the output future prediction, $X^+_1$ (completing the notation from the previous subsection). Therefore, incorporating our variational lower bound from eq.~\eqref{eq:elbo}, the optimization objective of learning our model becomes: 
% \begin{align}
%     \min_\theta \mathcal{L} - \lambda I(Z_1, X^+_1) 
% \end{align}
% As noted by \citet{chen2016infogan}, in practice, maximizing the mutual information term directly is hard, since it requires access to the posterior $\mathcal{P}(Z|X^+)$. We can instead lower bound the information term using Variational Information Maximization \cite{agakov2004algorithm}. As shown by \citet{chen2016infogan}, the lower bound can be written as:
% \begin{align}
%     \begin{split}
%         L_I(f, Q) &= \mathbb{E}_{Z_1\sim P(Z_1),X^+_1\sim f(Z, X^-)}[\log Q(Z_1|X^+)] + H(Z_1) \leq \\ 
%         &\leq I(Z_1, f(Z, X^-)) = I(Z_1, X^+_1)  = H(z_1) - H(Z_1|f(Z, X^-))        
%     \end{split}
% \end{align}


% Currently, our agent predicts $X^+ \sim P(X^+|X^-, Y^-; Z)$ and the opponent predicts $Y^+ \sim P(Y^+|X^-, Y^-, X^+; W) = \frac{P(Y^+, X^+|X^-, Y^-; W)}{P(X^+|X^-, Y^-)} $


% Multi agent dynamics:
% $x_{t+1},y_{t+1} = f(x_t, y_t, u_t, v_t, w_t)$, where $w_t$ is noise. 
% This is equivalent to writing $P(x_{t+1},y_{t+1}|x_t, y_t, u_t, v_t)$. If $v_t \sim \pi_y$, then
% $P(x_{t+1},y_{t+1}|x_t, y_t, u_t) = \sum_{v_t}P(x_{t+1},y_{t+1}|x_t, y_t, u_t, v_t)\pi_y(v_t)$. 

% And $P(x_{t+1},y_{t+1}|x_t, y_t, u_t) = P(y_{t+1}|x_{t+1},x_t, y_t, u_t)P(x_{t+1}|x_t, y_t, u_t)$.

% Assuming that actions only control single agents, $P(y_{t+1}|x_{t+1},x_t, y_t, u_t) = P(y_{t+1}|x_{t+1},x_t, y_t)$, so 

% $$P(x_{t+1},y_{t+1}|x_t, y_t, u_t) = P(y_{t+1}|x_{t+1},x_t, y_t)P(x_{t+1}|x_t, y_t, u_t)$$
%%%%%%%%%%%%%%%%%
